The Most Metal-Poor Stars. I. Discovery, Data, and Atmospheric Parameters

We report the discovery of 34 stars in the Hamburg/ESO Survey for metal-poor stars and the Sloan Digital Sky Survey that have [Fe/H] < -3.0. Their median and minimum abundances are [Fe/H] = -3.1 and -4.1, respectively, while 10 stars have [Fe/H] < -3.5. High-resolution, high-S/N spectroscopic data - equivalent widths and radial velocities - are presented for these stars, together with an additional four objects previously reported or currently being investigated elsewhere. We have determined the atmospheric parameters, effective temperature (Teff) and surface gravity (logg), which are critical in the determination of the chemical abundances and the evolutionary status of these stars. Three techniques were used to derive these parameters. Spectrophotometric fits to model atmosphere fluxes were used to derive Teff, logg, and an estimate of E(B-V); Halpha, Hbeta, and Hgamma profile fitting to model atmosphere results provided the second determination of Teff and logg; and finally, we used an empirical Teff-calibrated Hdelta index, for the third, independent Teff determination. The three values of Teff are in good agreement, although the profile fitting may yield systematically cooler Teff values, by ~100K. This collective data set will be analyzed in future papers in the present series to utilize the most metal-poor stars as probes of conditions in the early Universe.

==> tab3.tex <==
\begin{center}                                                                                                          
\begin{deluxetable}{cccrrrrrrrrrr}                                                                                      
\tabletypesize{\tiny}                                                                                                   
\tablecolumns{13}                                                                                                       
\tablewidth{0pt}                                                                                                        
\rotate                                                                                                                 
\tablecaption{\label{Tab:table3} ATOMIC DATA AND EQUIVALENT WIDTHS (m{\AA}) FOR PROGRAM STARS }                       
\tablehead{                                                                                                             
\colhead{Wavelength} & {Species} & {$\chi$} & {log$gf$} & {52972-1213} & {53327-2044} & {53436-1996} & {54142-2667} & {BS~16545} & {CS~30336} & {HE~0049} & {HE~0057} & {HE~0102} \\
{(\AA)}   & &{($\rm eV$)} &                             & {-507}       & {-515}       & {-093}       & {-094}       & {-089}     & {-049}     & {--3948}  & {--5959}  & {--1213} \\
{(1)}     & {(2)} & {(3)} & {(4)}                       & {(5)}        & {(6)}        & {(7)}        & {(8)}        & {(9)}      & {(10)}     & {(11)}    & {(12)}    & {(13)}
}                                                                                                                       
\startdata                                                                                                              
$S/N$\tablenotemark{a}  &  &  &  &    28 &     51 &    129 &     47 &    180 &    126 &    149 &     91 &     81 \\
W(min)\,(m{\AA})  &  &  &  &    12 &      7 &      6 &      8 &      5 &      6 &      6 &      6 &      5 \\\\
 5889.95 &   11.0 &   0.00 &    0.11 &  183.0 &    ...  &    ...  &    ...  &   20.2  &   70.4  &   10.6  &  156.0  &    ...  \\
 5895.92 &   11.0 &   0.00 &   $-$0.19 &  105.0  &   17.8  &   10.9  &    ...  &   11.6  &   50.6  &   12.6  &  129.0  &   32.7  \\
 3829.36 &   12.0 &   2.71 &   $-$0.21 &   93.0  &   65.4  &    ...  &   88.7  &    ...  &   93.6  &   43.8  &   86.1  &   78.5  \\
 3832.30 &   12.0 &   2.71 &    0.15 &    ...  &    ...  &    ...  &    ...  &    ...  &  106.5  &    ...  &  106.5  &    ...  \\
 3838.29 &   12.0 &   2.72 &    0.41 &    ...  &    ...  &    ...  &    ...  &    ...  &  117.5  &    ...  &  109.5  &    ...  \\
 4571.10 &   12.0 &   0.00 &   $-$5.39 &    ...  &    ...  &    ...  &    ...  &    ...  &    5.3  &    ...  &    ...  &    ...  \\
 5172.68 &   12.0 &   2.71 &   $-$0.38 &   90.1  &   71.9  &   57.8  &   78.8  &   59.8  &   94.8  &   45.6  &   85.4  &   77.7  \\
 5183.60 &   12.0 &   2.72 &   $-$0.16 &  112.0  &   81.4  &   66.3  &  106.5  &   75.3  &  110.5  &   56.3  &  117.5  &   97.8  \\
 5528.41 &   12.0 &   4.34 &   $-$0.34 &    ...  &    ...  &    ...  &    ...  &    5.8  &   11.2  &    ...  &    6.8  &    4.7  \\
 3944.01 &   13.0 &   0.00 &   $-$0.64 &    ...  &    ...  &    ...  &   26.2  &    ...  &   44.0  &    ...  &   56.6  &   22.4  \\
 3961.52 &   13.0 &   0.01 &   $-$0.34 &    ...  &   38.0  &    ...  &   31.0  &    ...  &   53.8  &    ...  &    ...  &   35.2  \\
 3905.52 &   14.0 &   1.91 &   $-$1.09 &    ...  &   60.8  &    ...  &   58.9  &    ...  &  108.0  &   23.0  &   84.7  &   69.2  \\
 4226.73 &   20.0 &   0.00 &    0.24 &   98.8  &   67.9  &   67.7  &   85.8  &   75.2  &  102.5 &   46.5  &   88.9  &   89.9  \\
 4283.01 &   20.0 &   1.89 &   $-$0.22 &    ...  &    ...  &    ...  &    ...  &    ...  &    8.1  &    ...  &    ...  &    7.1  \\
 4318.65 &   20.0 &   1.90 &   $-$0.21 &    ...  &    ...  &    ...  &    ...  &    ...  &    8.1  &    ...  &    7.6  &    7.7  \\
 4435.68 &   20.0 &   1.89 &   $-$0.52 &    ...  &    ...  &    ...  &    8.4  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4454.78 &   20.0 &   1.90 &    0.26 &    ...  &    ...  &    ...  &   13.0  &   10.4  &   13.1  &    ...  &   11.5  &   16.2  \\
 5588.75 &   20.0 &   2.52 &    0.21 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    9.8  \\
 5857.45 &   20.0 &   2.93 &    0.23 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 6122.22 &   20.0 &   1.89 &   $-$0.32 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   10.6  &    ...  \\
 6162.17 &   20.0 &   1.90 &   $-$0.09 &    ...  &    ...  &    ...  &    ...  &    7.2  &    ...  &    ...  &    ...  &    ...  \\
 6439.08 &   20.0 &   2.52 &    0.47 &    ...  &    ...  &    ...  &    ...  &    7.2  &    ...  &    ...  &    8.6  &    ...  \\
 4246.82 &   21.1 &   0.31 &    0.24 &    ...  &    5.2  &   12.6  &   32.2  &   12.0  &   65.3  &    ...  &   24.5  &   25.6  \\
 4314.08 &   21.1 &   0.62 &   $-$0.10 &    ...  &    ...  &    ...  &   12.4  &    ...  &   25.2  &    ...  &    7.2  &    6.1  \\
 3998.64 &   22.0 &   0.05 &   $-$0.06 &    ...  &    ...  &    ...  &    ...  &    ...  &   11.5  &    ...  &    8.6  &    8.1  \\
 4533.24 &   22.0 &   0.85 &    0.48 &    ...  &    ...  &    ...  &    ...  &    ...  &    4.2  &    ...  &    ...  &    ...  \\
 4981.73 &   22.0 &   0.84 &    0.50 &    ...  &    ...  &    ...  &   11.7  &    ...  &    ...  &    ...  &    ...  &    6.1  \\
 4991.07 &   22.0 &   0.84 &    0.38 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    6.5  \\
 4999.50 &   22.0 &   0.83 &    0.25 &    ...  &    ...  &    ...  &    7.8  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5192.97 &   22.0 &   0.02 &   $-$1.01 &    ...  &    ...  &    ...  &    ...  &    ...  &   12.9\tablenotemark{b} &    ...  &    ...  &    ...  \\
 3759.30 &   22.1 &   0.61 &    0.27 &   70.0  &   44.1  &    ...  &   91.4  &    ...  &  113.0  &   43.6  &   79.2  &   82.9  \\
 3761.32 &   22.1 &   0.57 &    0.17 &   61.8  &   37.0  &    ...  &   81.6  &    ...  &   96.2  &   56.0  &   85.8  &   76.8  \\
 3913.47 &   22.1 &   1.12 &   $-$0.41 &   31.1  &   11.4  &    ...  &   38.9  &    ...  &   52.5  &   15.8  &   34.5  &   34.8  \\
 4012.39 &   22.1 &   0.57 &   $-$1.75 &    ...  &    ...  &    ...  &    ...  &    ...  &   27.8  &    ...  &    ...  &   10.1  \\
 4028.34 &   22.1 &   1.89 &   $-$0.99 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4290.22 &   22.1 &   1.16 &   $-$0.93 &    ...  &    ...  &    ...  &   13.1  &    7.8  &   27.0  &    6.1  &   14.6  &   14.8  \\
 4300.05 &   22.1 &   1.18 &   $-$0.49 &    ...  &    ...  &    7.3  &    ...  &   18.3  &   39.8  &    7.2  &   18.2  &   27.8  \\
 4395.03 &   22.1 &   1.08 &   $-$0.51 &    ...  &    ...  &   14.1  &   35.0  &   19.2  &   47.8  &   11.3  &   28.7  &   30.0  \\
 4399.77 &   22.1 &   1.24 &   $-$1.22 &    ...  &    ...  &    ...  &    ...  &    3.4  &   11.6  &    ...  &    ...  &    ...  \\
 4417.72 &   22.1 &   1.16 &   $-$1.23 &    ...  &    ...  &    ...  &    ...  &    4.3  &   16.0  &    ...  &   10.1  &    ...  \\
 4443.79 &   22.1 &   1.08 &   $-$0.70 &    ...  &    ...  &   11.4  &   19.5  &   13.9  &   45.5  &    8.0  &   22.3  &    ...  \\
 4450.48 &   22.1 &   1.08 &   $-$1.51 &    ...  &    ...  &    ...  &   11.4  &    ...  &   12.2  &    ...  &    ...  &    ...  \\
 4464.45 &   22.1 &   1.16 &   $-$1.81 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4468.51 &   22.1 &   1.13 &   $-$0.60 &   28.3  &    ...  &    7.8  &   31.9  &   13.8  &   43.2  &    7.1  &   21.5  &   25.0  \\
 4501.27 &   22.1 &   1.12 &   $-$0.76 &   23.7  &    ...  &    8.8  &    ...  &   12.1  &   39.4  &    ...  &   17.3  &   27.6  \\
 4533.97 &   22.1 &   1.24 &   $-$0.54 &    ...  &    ...  &    7.6  &   24.5  &   14.1  &   35.9  &    ...  &   23.5  &   21.5  \\
 4563.76 &   22.1 &   1.22 &   $-$0.79 &    ...  &    ...  &    5.4  &   18.2  &   10.9  &   29.2  &    ...  &   17.8  &   13.6  \\
 4571.97 &   22.1 &   1.57 &   $-$0.23 &    ...  &    ...  &    9.4  &   30.4  &   14.4  &   33.7  &    ...  &   15.5  &   18.0  \\
 5185.91 &   22.1 &   1.89 &   $-$1.37 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5188.68 &   22.1 &   1.58 &   $-$1.05 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5226.54 &   22.1 &   1.57 &   $-$1.23 &    ...  &    ...  &    ...  &   53.5\tablenotemark{b} &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4254.33 &   24.0 &   0.00 &   $-$0.11 &   20.2  &    ...  &   13.1  &   26.8  &    8.8  &   38.4  &    6.2 &   17.3  &   21.5  \\
 4274.80 &   24.0 &   0.00 &   $-$0.23 &    ...  &    ...  &    9.9  &   21.4  &    9.3  &   32.9  &    ...  &   11.8  &   21.2  \\
 4289.72 &   24.0 &   0.00 &   $-$0.36 &    ...  &    ...  &    6.4  &   17.0  &    7.8  &   29.5  &    ...  &   18.1  &   16.4  \\
 5206.04 &   24.0 &   0.94 &    0.02 &    ...  &    ...  &    5.9  &    ...  &    ...  &   14.1  &    8.3  &    ...  &    ...  \\
 5208.42 &   24.0 &   0.94 &    0.16 &    ...  &    ...  &    ...  &    ...  &    ...  &   18.3  &    ...  &    ...  &   17.7  \\
 4030.75 &   25.0 &   0.00 &   $-$0.48 &    ...  &    ...  &    ...  &    ...  &    ...  &   28.7  &    ...  &    ...  &   11.5  \\
 4033.06 &   25.0 &   0.00 &   $-$0.62 &    ...  &    ...  &    ...  &   12.6  &    ...  &   25.8  &    ...  &    ...  &    7.1  \\
 4034.48 &   25.0 &   0.00 &   $-$0.81 &    ...  &    ...  &    ...  &    ...  &    ...  &   19.2  &    ...  &    ...  &    ...  \\
 3743.36 &   26.0 &   0.99 &   $-$0.79 &   45.4  &   29.3  &    ...  &    ...  &    ...  &    ...  &   18.0  &   54.3  &   52.7  \\
 3758.23 &   26.0 &   0.96 &   $-$0.03 &   69.9  &   67.0  &    ...  &   80.4  &    ...  &  110.5  &   46.8  &   93.1  &   84.4  \\
 3763.79 &   26.0 &   0.99 &   $-$0.24 &   72.7  &   57.1  &    ...  &   61.8  &    ...  &  104.5  &   33.1  &   75.1  &   74.6  \\
 3765.54 &   26.0 &   3.24 &    0.48 &    ...  &    ...  &    ...  &    ...  &    ...  &   27.8  &    ...  &   17.5  &   13.8  \\
 3767.19 &   26.0 &   1.01 &   $-$0.39 &    ...  &    ...  &    ...  &    ...  &    ...  &   92.7  &    ...  &   67.8  &   71.0  \\
 3786.68 &   26.0 &   1.01 &   $-$2.23 &    ...  &    ...  &    ...  &    ...  &    ...  &   27.7  &    ...  &    ...  &    8.8  \\
 3787.88 &   26.0 &   1.01 &   $-$0.86 &    ...  &   26.3  &    ...  &   43.3  &    ...  &   89.6  &   20.6  &   53.3  &   53.6  \\
 3805.34 &   26.0 &   3.30 &    0.31 &    ...  &    ...  &    ...  &    ...  &    ...  &   16.5  &    ...  &    ...  &    8.4  \\
 3815.84 &   26.0 &   1.48 &    0.24 &   79.5  &   55.8  &    ...  &   80.5  &    ...  &   97.7  &   42.8  &   71.8  &   75.6  \\
 3820.43 &   26.0 &   0.86 &    0.12 &   94.7  &   81.4  &    ...  &   86.4  &    ...  &  129.0  &   60.5  &   95.5  &   90.4  \\
 3824.44 &   26.0 &   0.00 &   $-$1.36 &   59.2  &   60.4  &    ...  &   73.8  &    ...  &  125.0  &   31.5  &   83.1  &   79.9  \\
 3825.88 &   26.0 &   0.91 &   $-$0.04 &   86.4  &   69.8  &    ...  &   82.8  &    ...  &  120.0  &   45.4  &   84.6  &   84.8  \\
 3827.82 &   26.0 &   1.56 &    0.06 &   65.8  &   46.5  &    ...  &   65.4  &    ...  &   88.3  &   31.4  &   57.0  &   61.2  \\
 3840.44 &   26.0 &   0.99 &   $-$0.51 &   62.7  &    ...  &    ...  &    ...  &    ...  &   91.6  &   26.8  &   72.2  &    ...  \\
 3849.97 &   26.0 &   1.01 &   $-$0.97 &   52.2  &   29.2  &    ...  &    ...  &    ...  &   86.1  &   16.5  &   57.9  &   50.1  \\
 3850.82 &   26.0 &   0.99 &   $-$1.73 &    ...  &    ...  &    ...  &    ...  &    ...  &   49.2  &    ...  &   30.6  &   16.5  \\
 3856.37 &   26.0 &   0.05 &   $-$1.29 &   73.2  &   63.0  &    ...  &   67.4  &    ...  &  125.5  &   36.5  &   82.6  &   79.2  \\
 3859.91 &   26.0 &   0.00 &   $-$0.71 &   85.4  &   87.8  &    ...  &   95.6  &    ...  &  142.0  &   63.1\tablenotemark{b}  &  104.5  &   92.9  \\
 3865.52 &   26.0 &   1.01 &   $-$0.98 &   39.1  &   21.5  &    ...  &   46.4  &    ...  &   86.1  &   13.4  &   48.6  &   47.7  \\
 3878.02 &   26.0 &   0.96 &   $-$0.91 &   44.7  &   28.0  &    ...  &   41.2  &    ...  &   92.4  &   17.5  &   52.6  &   49.4  \\
 3878.57 &   26.0 &   0.09 &   $-$1.38 &    ...  &   52.8  &    ...  &   66.3  &    ...  &  123.0  &   30.2  &   82.5  &   78.0  \\
 3886.28 &   26.0 &   0.05 &   $-$1.08 &    ...  &    ...  &    ...  &    ...  &    ...  &  128.5  &    ...  &   88.6  &    ...  \\
 3887.05 &   26.0 &   0.91 &   $-$1.14 &    ...  &    ...  &    ...  &    ...  &    ...  &   85.2  &    ...  &   49.0  &    ...  \\
 3895.66 &   26.0 &   0.11 &   $-$1.67 &    ...  &   43.2  &    ...  &   42.2  &    ...  &  109.0  &   18.5  &   70.4  &   56.5  \\
 3899.71 &   26.0 &   0.09 &   $-$1.53 &   58.2  &   50.5  &    ...  &   56.7  &    ...  &  110.0  &   23.2  &   76.0  &   66.2  \\
 3920.26 &   26.0 &   0.12 &   $-$1.75 &    ...  &   37.0  &    ...  &   49.1  &    ...  &   99.7  &   13.9  &   71.2  &   58.7  \\
 3922.91 &   26.0 &   0.05 &   $-$1.65 &   50.3  &   44.0  &    ...  &   59.5  &    ...  &  116.0  &   22.7  &   72.3  &   64.9  \\
 4005.24 &   26.0 &   1.56 &   $-$0.61 &   31.3  &   25.9  &    ...  &   42.8  &    ...  &   74.6  &   13.9  &   38.6  &   41.8  \\
 4045.81 &   26.0 &   1.48 &    0.28 &   68.2  &   60.3  &   58.8  &   74.1  &   63.1  &  102.5  &   47.3  &   72.8  &   77.2  \\
 4063.59 &   26.0 &   1.56 &    0.07 &   58.7  &   45.9  &   43.3  &   68.4  &   46.6  &   94.6  &   36.8  &   68.7  &   66.7  \\
 4071.74 &   26.0 &   1.61 &   $-$0.02 &   50.3  &   42.2  &   40.7  &   64.9  &   39.5  &   86.7  &   28.3  &   56.1  &   68.1  \\
 4076.63 &   26.0 &   3.21 &   $-$0.37 &    ...  &    ...  &    ...  &    9.2  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4132.06 &   26.0 &   1.61 &   $-$0.67 &   27.8  &    ...  &   18.7  &   35.9  &   16.2  &   62.1  &    8.8  &   31.0  &   31.5  \\
 4134.68 &   26.0 &   2.83 &   $-$0.49 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4143.87 &   26.0 &   1.56 &   $-$0.46 &   37.8  &   21.1  &   21.0  &   44.7  &   25.1  &   70.8  &   11.9  &   45.5  &   46.8  \\
 4147.67 &   26.0 &   1.48 &   $-$2.10 &    ...  &    ...  &    ...  &    ...  &    ...  &   11.0  &    ...  &    ...  &    ...  \\
 4156.80 &   26.0 &   2.83 &   $-$0.61 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    5.8  \\
 4181.76 &   26.0 &   2.83 &   $-$0.18 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4187.04 &   26.0 &   2.45 &   $-$0.55 &    ...  &    ...  &    ...  &    8.2  &    ...  &   20.1  &    ...  &    8.2  &   11.4  \\
 4187.80 &   26.0 &   2.42 &   $-$0.55 &    ...  &    ...  &    ...  &    ...  &    6.0  &   22.7  &    ...  &    6.8  &    ...  \\
 4191.43 &   26.0 &   2.47 &   $-$0.73 &    ...  &    ...  &    ...  &    ...  &    ...  &   12.9  &    ...  &    6.3  &    ...  \\
 4199.10 &   26.0 &   3.05 &    0.25 &    ...  &    ...  &    5.6 &   19.8  &    6.9  &   19.5  &    ...  &    9.9  &   13.1  \\
 4202.03 &   26.0 &   1.48 &   $-$0.70 &    ...  &   17.8  &   17.6  &   35.8  &   20.0  &   69.8  &   12.9  &   43.0  &   40.2  \\
 4222.21 &   26.0 &   2.45 &   $-$0.97 &   12.0 &    ...  &    ...  &    ...  &    ...  &    6.4  &    ...  &    6.6  &    ...  \\
 4227.43 &   26.0 &   3.33 &    0.23 &    ...  &    ...  &    ...  &    ...  &    6.9  &   15.1  &    ...  &    ...  &   10.4  \\
 4233.60 &   26.0 &   2.48 &   $-$0.60 &    ...  &    ...  &    ...  &    ...  &    ...  &   18.0  &    ...  &    ...  &   11.1  \\
 4250.12 &   26.0 &   2.47 &   $-$0.40 &    ...  &    ...  &    ...  &   17.2  &    6.2  &   26.4  &    5.2 &    8.9  &   16.2  \\
 4260.47 &   26.0 &   2.40 &   $-$0.02 &   32.2  &   18.4  &   13.6  &   37.2  &   16.8  &   46.1  &   10.8  &   32.0  &   35.8  \\
 4271.15 &   26.0 &   2.45 &   $-$0.35 &    ...  &    ...  &    ...  &    ...  &    5.8  &   27.7  &    ...  &   14.2  &   12.9  \\
 4271.76 &   26.0 &   1.48 &   $-$0.16 &    ...  &   50.2  &   41.9  &   62.0  &   42.6  &   91.0  &   31.9  &   63.3  &   63.6  \\
 4282.40 &   26.0 &   2.17 &   $-$0.82 &    ...  &    ...  &    ...  &    ...  &    4.4 &   18.7  &    ...  &    5.6 &   11.7  \\
 4325.76 &   26.0 &   1.61 &   $-$0.01 &    ...  &   43.8  &   39.7  &   63.0  &   42.3  &   88.3  &   29.6  &   61.2  &   58.8  \\
 4383.55 &   26.0 &   1.48 &    0.20 &   71.6  &   63.0  &   57.7  &   77.0  &   62.0  &  108.0  &   47.2  &   74.3  &   80.3  \\
 4404.75 &   26.0 &   1.56 &   $-$0.14 &   64.1  &   43.7  &   39.1  &   62.2  &   40.2  &   89.6  &   28.2  &   60.5  &   62.3  \\
 4415.12 &   26.0 &   1.61 &   $-$0.61 &    ...  &    ...  &   17.3  &   40.3  &   18.3  &   66.2  &   13.0  &   37.3  &   40.2  \\
 4442.34 &   26.0 &   2.20 &   $-$1.25 &    ...  &    ...  &    ...  &    ...  &    ...  &    7.1  &    ...  &    ...  &    ...  \\
 4447.72 &   26.0 &   2.22 &   $-$1.34 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4461.65 &   26.0 &   0.09 &   $-$3.20 &    ...  &    ...  &    ...  &    ...  &    ...  &   46.7  &    ...  &   10.8  &    ...  \\
 4466.55 &   26.0 &   2.83 &   $-$0.60 &    ...  &    ...  &    ...  &    ...  &    ...  &    9.2  &    ...  &    ...  &    ...  \\
 4489.74 &   26.0 &   0.12 &   $-$3.97 &    ...  &    ...  &    ...  &    ...  &    ...  &   12.7  &    ...  &    ...  &    ...  \\
 4494.56 &   26.0 &   2.20 &   $-$1.14 &    ...  &    ...  &    ...  &    ...  &    ...  &   13.8  &    ...  &    ...  &    7.3  \\
 4528.61 &   26.0 &   2.18 &   $-$0.82 &    ...  &    ...  &    ...  &    ...  &    3.7 &   21.9  &    ...  &    ...  &   11.1  \\
 4531.15 &   26.0 &   1.48 &   $-$2.15 &    ...  &    ...  &    ...  &    ...  &    ...  &   12.4  &    ...  &    ...  &    ...  \\
 4871.32 &   26.0 &   2.87 &   $-$0.36 &    ...  &    ...  &    ...  &    ...  &    ...  &   13.0  &    ...  &    ...  &    ...  \\
 4872.14 &   26.0 &   2.88 &   $-$0.57 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4891.49 &   26.0 &   2.85 &   $-$0.11 &    ...  &    ...  &    ...  &   18.6  &    ...  &   20.8  &    ...  &    8.9  &   12.8  \\
 4903.31 &   26.0 &   2.88 &   $-$0.93 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4918.99 &   26.0 &   2.87 &   $-$0.34 &    ...  &    ...  &    ...  &    ...  &    ...  &   10.6  &    ...  &    ...  &    ...  \\
 4920.50 &   26.0 &   2.83 &    0.07 &    ...  &    6.4 &    ...  &   13.0  &    9.1  &   26.5  &    ...  &   12.9  &   11.9  \\
 4939.69 &   26.0 &   0.86 &   $-$3.34 &    ...  &    ...  &    ...  &    ...  &    ...  &    6.0 &    ...  &    ...  &    ...  \\
 4994.13 &   26.0 &   0.92 &   $-$3.08 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5006.12 &   26.0 &   2.83 &   $-$0.62 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5041.76 &   26.0 &   1.49 &   $-$2.20 &    ...  &    ...  &    ...  &    ...  &    ...  &   11.1  &    ...  &    ...  &    ...  \\
 5051.64 &   26.0 &   0.92 &   $-$2.80 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   13.5\tablenotemark{b} &    ...  \\
 5083.34 &   26.0 &   0.96 &   $-$2.96 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    5.2\tablenotemark{b} \\
 5123.72 &   26.0 &   1.01 &   $-$3.07 &    ...  &    ...  &    ...  &    ...  &    ...  &   17.0\tablenotemark{b} &    ...  &    ...  &    ...  \\
 5127.36 &   26.0 &   0.92 &   $-$3.31 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5150.84 &   26.0 &   0.99 &   $-$3.04 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5166.28 &   26.0 &   0.00 &   $-$4.20 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5171.60 &   26.0 &   1.49 &   $-$1.79 &    ...  &    ...  &    ...  &    ...  &    ...  &   30.6  &    ...  &    ...  &   12.1  \\
 5191.46 &   26.0 &   3.04 &   $-$0.55 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5192.34 &   26.0 &   3.00 &   $-$0.42 &    ...  &    ...  &    ...  &   10.6  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5194.94 &   26.0 &   1.56 &   $-$2.09 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5216.27 &   26.0 &   1.61 &   $-$2.15 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5232.94 &   26.0 &   2.94 &   $-$0.06 &    ...  &    ...  &    ...  &    ...  &    ...  &   13.4  &    ...  &    ...  &    8.4  \\
 5266.56 &   26.0 &   3.00 &   $-$0.39 &    ...  &    ...  &    ...  &    ...  &    ...  &    9.4  &    ...  &    ...  &    ...  \\
 5269.54 &   26.0 &   0.86 &   $-$1.32 &   28.0  &   27.1  &   16.8  &   37.0  &   18.7  &  104.5  &   11.4  &   60.6  &   44.2  \\
 5281.79 &   26.0 &   3.04 &   $-$0.83 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   11.8\tablenotemark{b} \\
 5283.62 &   26.0 &   3.24 &   $-$0.52 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5324.18 &   26.0 &   3.21 &   $-$0.24 &    ...  &    ...  &    ...  &    ...  &    ...  &   13.2  &    ...  &    ...  &    ...  \\
 5328.04 &   26.0 &   0.92 &   $-$1.47 &   32.9  &   21.7  &   11.6  &   28.9  &   13.8  &   94.8  &   14.0  &   33.9  &   38.9  \\
 5328.53 &   26.0 &   1.56 &   $-$1.85 &    ...  &    ...  &    ...  &    ...  &    ...  &   25.0  &    ...  &    ...  &    ...  \\
 5371.49 &   26.0 &   0.96 &   $-$1.65 &   25.0  &   10.6  &    8.4  &   20.6  &    9.6  &   82.7  &    ...  &   33.6  &   25.3  \\
 5397.13 &   26.0 &   0.92 &   $-$1.99 &    ...  &    ...  &    5.4 &   20.2  &    ...  &   68.3  &    ...  &   23.0  &   18.1  \\
 5405.78 &   26.0 &   0.99 &   $-$1.84 &    ...  &    ...  &    ...  &    ...  &    ...  &   65.9  &    ...  &   22.4  &   28.4  \\
 5429.70 &   26.0 &   0.96 &   $-$1.88 &    ...  &   13.5  &    ...  &    ...  &    ...  &   72.5  &    ...  &   23.1  &   18.2  \\
 5434.52 &   26.0 &   1.01 &   $-$2.12 &    ...  &    ...  &    ...  &    ...  &    ...  &   46.3  &    ...  &    ...  &   11.8  \\
 5446.92 &   26.0 &   0.99 &   $-$1.91 &    ...  &    ...  &    ...  &    ...  &    6.1  &   59.2  &    ...  &   26.1  &   19.6  \\
 5455.61 &   26.0 &   1.01 &   $-$2.09 &    ...  &    ...  &    ...  &    ...  &    ...  &   46.5  &    ...  &    ...  &    ...  \\
 5497.52 &   26.0 &   1.01 &   $-$2.85 &    ...  &    ...  &    ...  &    ...  &    ...  &   15.1  &    ...  &    ...  &    ...  \\
 5501.47 &   26.0 &   0.96 &   $-$3.05 &    ...  &    ...  &    ...  &    ...  &    ...  &   10.4  &    ...  &    ...  &    ...  \\
 5506.78 &   26.0 &   0.99 &   $-$2.80 &    ...  &    ...  &    ...  &    ...  &    ...  &   19.5  &    9.9\tablenotemark{b} &    ...  &    ...  \\
 5572.84 &   26.0 &   3.40 &   $-$0.31 &    ...  &    6.9\tablenotemark{b} &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5586.76 &   26.0 &   3.37 &   $-$0.14 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5615.64 &   26.0 &   3.33 &   $-$0.14 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 6136.62 &   26.0 &   2.45 &   $-$1.40 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 6137.69 &   26.0 &   2.59 &   $-$1.40 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 6191.56 &   26.0 &   2.43 &   $-$1.42 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 6230.72 &   26.0 &   2.56 &   $-$1.28 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 6252.56 &   26.0 &   2.40 &   $-$1.69 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 6393.60 &   26.0 &   2.43 &   $-$1.58 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 6494.98 &   26.0 &   2.40 &   $-$1.27 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4178.86 &   26.1 &   2.58 &   $-$2.50 &    ...  &    ...  &    ...  &    ...  &    ...  &    6.4  &    ...  &    ...  &    ...  \\
 4233.17 &   26.1 &   2.58 &   $-$1.90 &    ...  &    ...  &    ...  &   19.0  &    ...  &   19.0  &    5.9 &    ...  &   12.0  \\
 4508.29 &   26.1 &   2.86 &   $-$2.25 &    ...  &    ...  &    ...  &    ...  &    ...  &    5.8 &    ...  &    ...  &    ...  \\
 4520.22 &   26.1 &   2.81 &   $-$2.60 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    5.8  \\
 4522.63 &   26.1 &   2.84 &   $-$2.03 &    ...  &    ...  &    ...  &    ...  &    ...  &    6.3  &    ...  &    ...  &    ...  \\
 5197.58 &   26.1 &   3.23 &   $-$2.23 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5234.63 &   26.1 &   3.22 &   $-$2.15 &    ...  &    ...  &    ...  &    ...  &    ...  &    7.1  &    ...  &    ...  &    ...  \\
 3845.46 &   27.0 &   0.92 &    0.01 &   15.9  &    ...  &    ...  &    ...  &    ...  &   33.7  &    ...  &    ...  &   11.9  \\
 3995.30 &   27.0 &   0.92 &   $-$0.22 &    ...  &    ...  &    ...  &    ...  &    ...  &   26.0  &    ...  &    ...  &    ...  \\
 4118.77 &   27.0 &   1.05 &   $-$0.49 &    ...  &    ...  &    ...  &    ...  &    ...  &   17.2  &    ...  &    ...  &    9.4  \\
 4121.31 &   27.0 &   0.92 &   $-$0.32 &    ...  &    ...  &    ...  &    ...  &    ...  &   32.5  &    ...  &    ...  &    ...  \\
 3807.14 &   28.0 &   0.42 &   $-$1.18 &    ...  &   11.5  &    ...  &    ...  &    ...  &   64.9  &    ...  &   31.8  &   25.0  \\
 3858.29 &   28.0 &   0.42 &   $-$0.97 &   31.6  &   19.8  &    ...  &   21.0  &    ...  &   76.9  &   12.7  &   45.2  &   32.6  \\
 5476.90 &   28.0 &   1.83 &   $-$0.89 &    ...  &    ...  &    ...  &    ...  &    ...  &   12.4  &    ...  &    ...  &    ...  \\
 4077.71 &   38.1 &   0.00 &    0.16 &   84.7  &   59.5  &   38.5  &   12.3  &   30.5  &   24.2  &    5.9  &   15.9  &   47.0  \\
 4215.52 &   38.1 &   0.00 &   $-$0.16 &   76.2  &   46.5  &   40.0  &   10.4  &   18.7  &   20.6  &    ...  &   10.4  &   30.9  \\
 4554.03 &   56.1 &   0.00 &    0.16 &   91.8  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    8.8  &    ...  \\
 4934.08 &   56.1 &   0.00 &   $-$0.15 &   85.4  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 6141.73 &   56.1 &   0.70 &   $-$0.08 &   39.9  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 6496.91 &   56.1 &   0.60 &   $-$0.38 &   48.3  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
\enddata                                                                                                                
\tablenotetext{a}{$S/N$ per $\sim$0.17\,{\AA}~pixel at 4500\,{\AA}}                                                      
\tablenotetext{b}{These lines produce discrepant abundances and are not included in the results reported in Paper II}   
\end{deluxetable}                                                                                                       

\end{center}                                                                                                          



==> tab4.tex <==
\begin{center}                                                                                                          
\begin{deluxetable}{cccrrrrrrrrrrr}                                                                                     
\tabletypesize{\tiny}                                                                                                   
\tablecolumns{14}                                                                                                       
\tablewidth{0pt}                                                                                                        
\rotate                                                                                                                 
\tablecaption{\label{Tab:table4} ATOMIC DATA AND EQUIVALENT WIDTHS (m{\AA}) FOR PROGRAM STARS}                       
\tablehead{                                                                                                             
\colhead{Wavelength} & {Species} & {$\chi$} & {log$gf$} & {HE~0146} & {HE~0207} & {HE~0228} & {HE~0231} & {HE~0253} & {HE~0314} & {HE~0355} & {HE~0945} & {HE~1055} & {HE~1116} \\
{(\AA)}   & &{($\rm eV$)} &                              & {--1548} & {--1423}  & {--4047}  & {--6025}  & {--1331}  & {--1739}  & {--3728}  & {--1435}  & {+0104 }  & {--0054} \\
{(1)} & {(2)} & {(3)} & {(4)}                            & {(5)}    & {(6)}     & {(7)}     & {(8)}     & {(9)}     & {(10)}    & {(11)}    & {(12)}    & {(13)}    & {(14)}
}                                                                                                                       
\startdata                                                                                                              
$S/N$\tablenotemark{a}  &  &  &  &    34 &     23 &    118 &     42 &     41 &     43 &     29 &    158 &     49 &    128 \\
W(min)\,(m{\AA})  &  &  &  &    14 &     13 &      6 &     13 &     10 &      9 &     20 &      5 &      9 &      7 \\\\
 5889.95 &   11.0 &   0.00 &    0.11 &  186.0  &  138.5  &    ...  &   44.2  &   45.1  &   29.9  &    ...  &    ...  &   67.1  &   16.4  \\
 5895.92 &   11.0 &   0.00 &   $-$0.19 &  154.5  &    ...  &    ...  &   37.7  &   23.4  &    ...  &    ...  &    ...  &   39.6  &   10.6  \\
 3829.36 &   12.0 &   2.71 &   $-$0.21 &    ...  &    ...  &   43.2  &  100.2  &   88.8  &   78.4  &    ...  &    ...  &   98.1  &   55.0  \\
 3832.30 &   12.0 &   2.71 &    0.15 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 3838.29 &   12.0 &   2.72 &    0.41 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4571.10 &   12.0 &   0.00 &   $-$5.39 &   60.3  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5172.68 &   12.0 &   2.71 &   $-$0.38 &  194.5  &  162.0  &   51.7  &   89.7  &   94.8  &   78.1  &    ...  &   27.6  &  109.5  &   51.3  \\
 5183.60 &   12.0 &   2.72 &   $-$0.16 &    ...  &  179.5  &   56.5  &  118.0  &   99.7  &   86.9  &    ...  &   39.1  &  120.0  &   67.7  \\
 5528.41 &   12.0 &   4.34 &   $-$0.34 &   66.1  &   58.7  &    ...  &   20.5  &   15.1  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 3944.01 &   13.0 &   0.00 &   $-$0.64 &    ...  &    ...  &    ...  &   24.6  &   24.4  &    ...  &    ...  &    ...  &   37.3  &    ...  \\
 3961.52 &   13.0 &   0.01 &   $-$0.34 &  132.0  &  123.0  &    ...  &   30.9  &   39.0  &   29.0  &    ...  &    ...  &   46.2  &    ...  \\
 3905.52 &   14.0 &   1.91 &   $-$1.09 &    ...  &    ...  &   35.8  &   58.6  &   62.5  &   53.8  &   44.0  &    ...  &   94.2  &    ...  \\
 4226.73 &   20.0 &   0.00 &    0.24 &  143.5  &    ...  &   63.2  &   96.2  &  110.5  &   92.6  &   73.9  &   50.5  &  109.0  &   70.1  \\
 4283.01 &   20.0 &   1.89 &   $-$0.22 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   11.8  &    ...  \\
 4318.65 &   20.0 &   1.90 &   $-$0.21 &    ...  &   43.4  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   14.5  &    ...  \\
 4435.68 &   20.0 &   1.89 &   $-$0.52 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4454.78 &   20.0 &   1.90 &    0.26 &    ...  &    ...  &    ...  &   21.9  &   25.2  &    ...  &    ...  &    5.2  &   29.0  &    7.8  \\
 5588.75 &   20.0 &   2.52 &    0.21 &    ...  &   32.9  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5857.45 &   20.0 &   2.93 &    0.23 &    ...  &   16.8  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 6122.22 &   20.0 &   1.89 &   $-$0.32 &    ...  &   43.5  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 6162.17 &   20.0 &   1.90 &   $-$0.09 &   36.2  &   47.3  &    ...  &    ...  &   14.2  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 6439.08 &   20.0 &   2.52 &    0.47 &    ...  &   35.7  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4246.82 &   21.1 &   0.31 &    0.24 &    ...  &    ...  &    ...  &   21.0  &   37.8  &   23.0  &    ...  &    4.4  &   32.8  &    9.9  \\
 4314.08 &   21.1 &   0.62 &   $-$0.10 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    9.0  &    ...  \\
 3998.64 &   22.0 &   0.05 &   $-$0.06 &   28.0  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4533.24 &   22.0 &   0.85 &    0.48 &    ...  &   22.0  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4981.73 &   22.0 &   0.84 &    0.50 &   23.0  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4991.07 &   22.0 &   0.84 &    0.38 &   30.3  &   20.6  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4999.50 &   22.0 &   0.83 &    0.25 &   14.2  &   26.8  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5192.97 &   22.0 &   0.02 &   $-$1.01 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 3759.30 &   22.1 &   0.61 &    0.27 &    ...  &    ...  &   50.5  &    ...  &   94.6  &   80.6  &   69.8  &    ...  &   86.8  &    ...  \\
 3761.32 &   22.1 &   0.57 &    0.17 &    ...  &  112.0  &   48.8  &    ...  &   85.4  &   81.5  &    ...  &    ...  &   84.8  &    ...  \\
 3913.47 &   22.1 &   1.12 &   $-$0.41 &    ...  &    ...  &   12.6  &   30.2  &   37.7  &   36.5  &    ...  &    ...  &   47.6  &    ...  \\
 4012.39 &   22.1 &   0.57 &   $-$1.75 &   72.4  &    ...  &    ...  &    ...  &   12.7  &    ...  &    ...  &    ...  &   14.5  &    ...  \\
 4028.34 &   22.1 &   1.89 &   $-$0.99 &   32.0  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4290.22 &   22.1 &   1.16 &   $-$0.93 &    ...  &    ...  &    ...  &   19.1  &    ...  &    ...  &    ...  &    ...  &   21.5  &    ...  \\
 4300.05 &   22.1 &   1.18 &   $-$0.49 &    ...  &    ...  &   10.0  &   24.8  &   29.2  &   23.5  &   32.7  &    ...  &   43.5  &    9.5  \\
 4395.03 &   22.1 &   1.08 &   $-$0.51 &    ...  &    ...  &   12.1  &   45.9  &   37.8  &   29.1  &   48.7  &    4.4  &   40.2  &   10.2  \\
 4399.77 &   22.1 &   1.24 &   $-$1.22 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   15.9  &    ...  \\
 4417.72 &   22.1 &   1.16 &   $-$1.23 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   12.4  &    ...  \\
 4443.79 &   22.1 &   1.08 &   $-$0.70 &   93.1  &   68.2  &    6.4  &    ...  &   26.1  &   21.8  &    ...  &    ...  &   36.2  &    8.6  \\
 4450.48 &   22.1 &   1.08 &   $-$1.51 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4464.45 &   22.1 &   1.16 &   $-$1.81 &    ...  &   43.2  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4468.51 &   22.1 &   1.13 &   $-$0.60 &   95.4  &    ...  &    6.2  &   29.5  &   28.4  &   23.8  &   22.0  &    ...  &   40.1  &    8.1  \\
 4501.27 &   22.1 &   1.12 &   $-$0.76 &   86.9  &   68.3  &    ...  &    ...  &    ...  &   26.5  &    ...  &    ...  &   26.0  &    9.0  \\
 4533.97 &   22.1 &   1.24 &   $-$0.54 &   85.4  &  103.8 &    ...  &   31.4  &    ...  &   16.3  &    ...  &    ...  &   32.7  &    7.6  \\
 4563.76 &   22.1 &   1.22 &   $-$0.79 &   65.7  &   71.1  &    ...  &   26.7  &   21.9  &   13.7  &    ...  &    ...  &   21.5  &    9.3  \\
 4571.97 &   22.1 &   1.57 &   $-$0.23 &   76.2  &   90.3  &    ...  &   29.9  &    ...  &   18.0  &    ...  &    5.9  &   21.9  &    8.1  \\
 5185.91 &   22.1 &   1.89 &   $-$1.37 &   13.9  &   11.8  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5188.68 &   22.1 &   1.58 &   $-$1.05 &   36.8  &   42.4  &    ...  &   33.6\tablenotemark{b} &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5226.54 &   22.1 &   1.57 &   $-$1.23 &   43.2  &   39.3  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4254.33 &   24.0 &   0.00 &   $-$0.11 &   82.2  &   98.5  &    6.1  &    ...  &   21.3  &   20.1  &    ...  &    4.9  &   34.6  &   13.1  \\
 4274.80 &   24.0 &   0.00 &   $-$0.23 &    ...  &    ...  &    6.1  &   22.6  &   23.4  &   17.7  &    ...  &    5.6  &   31.9  &    7.7  \\
 4289.72 &   24.0 &   0.00 &   $-$0.36 &    ...  &    ...  &    ...  &    ...  &   20.2  &    ...  &    ...  &    3.0  &   14.0  &    6.7  \\
 5206.04 &   24.0 &   0.94 &    0.02 &   46.0  &   55.2  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5208.42 &   24.0 &   0.94 &    0.16 &   56.7  &   67.9  &    ...  &    ...  &    ...  &   12.4  &    ...  &    ...  &   15.6  &    5.4  \\
 4030.75 &   25.0 &   0.00 &   $-$0.48 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   20.0  &    ...  \\
 4033.06 &   25.0 &   0.00 &   $-$0.62 &   88.8  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    9.9  &    ...  \\
 4034.48 &   25.0 &   0.00 &   $-$0.81 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 3743.36 &   26.0 &   0.99 &   $-$0.79 &    ...  &    ...  &    ...  &    ...  &   42.5  &   42.1  &    ...  &    ...  &   65.8  &    ...  \\
 3758.23 &   26.0 &   0.96 &   $-$0.03 &    ...  &    ...  &    ...  &    ...  &   86.2  &   81.7  &    ...  &    ...  &   89.6  &    ...  \\
 3763.79 &   26.0 &   0.99 &   $-$0.24 &    ...  &    ...  &   41.8  &    ...  &   63.1  &   63.0  &    ...  &    ...  &   76.2  &    ...  \\
 3765.54 &   26.0 &   3.24 &    0.48 &   43.8  &   55.2  &    ...  &    ...  &   17.9  &    ...  &    ...  &    ...  &   22.0  &    ...  \\
 3767.19 &   26.0 &   1.01 &   $-$0.39 &    ...  &  106.0  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   76.7  &    ...  \\
 3786.68 &   26.0 &   1.01 &   $-$2.23 &   56.9  &   58.5  &    ...  &    ...  &    ...  &   10.9  &    ...  &    ...  &    ...  &    ...  \\
 3787.88 &   26.0 &   1.01 &   $-$0.86 &  117.0  &   84.7  &    ...  &    ...  &   51.8  &   45.0  &    ...  &    ...  &   66.0  &   59.3  \\
 3805.34 &   26.0 &   3.30 &    0.31 &   36.1  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   15.5  &    ...  \\
 3815.84 &   26.0 &   1.48 &    0.24 &    ...  &    ...  &   43.6  &    ...  &   88.9  &   79.6  &   73.2  &    ...  &   86.4  &    ...  \\
 3820.43 &   26.0 &   0.86 &    0.12 &    ...  &    ...  &   66.2  &    ...  &   91.7  &   88.0  &    ...  &    ...  &  100.7  &   83.3  \\
 3824.44 &   26.0 &   0.00 &   $-$1.36 &    ...  &    ...  &   27.7  &   68.2  &   74.1  &   64.8  &    ...  &    ...  &   77.1  &   52.2  \\
 3825.88 &   26.0 &   0.91 &   $-$0.04 &    ...  &    ...  &   51.0  &   66.1\tablenotemark{b} &   74.7  &   73.8  &   64.6  &    ...  &   89.2  &   59.0  \\
 3827.82 &   26.0 &   1.56 &    0.06 &    ...  &    ...  &   30.8  &    ...  &   68.2  &   59.2  &    ...  &    ...  &   73.6  &   36.8  \\
 3840.44 &   26.0 &   0.99 &   $-$0.51 &    ...  &  117.0  &   28.6  &   38.1\tablenotemark{b} &    ...  &    ...  &    ...  &    ...  &   69.2  &    ...  \\
 3849.97 &   26.0 &   1.01 &   $-$0.97 &    ...  &    ...  &    ...  &   59.0  &   51.0  &   51.3  &    ...  &    ...  &   61.0  &   39.8  \\
 3850.82 &   26.0 &   0.99 &   $-$1.73 &    ...  &    ...  &    ...  &    ...  &    ...  &   15.6  &    ...  &    ...  &   24.5  &   19.6  \\
 3856.37 &   26.0 &   0.05 &   $-$1.29 &    ...  &    ...  &   38.2  &  100.5\tablenotemark{b} &   65.6  &   70.5  &   37.6  &    ...  &   80.3  &   52.9  \\
 3859.91 &   26.0 &   0.00 &   $-$0.71 &    ...  &    ...  &   66.1  &  104.5  &   98.8  &   86.8  &   74.1  &    ...  &  107.0  &   67.5  \\
 3865.52 &   26.0 &   1.01 &   $-$0.98 &    ...  &    ...  &    ...  &    ...  &   45.8  &   35.2  &    ...  &    ...  &   54.0  &   28.9  \\
 3878.02 &   26.0 &   0.96 &   $-$0.91 &    ...  &    ...  &   11.6  &   51.5  &   48.2  &   36.3  &    ...  &    ...  &   59.3  &   31.6  \\
 3878.57 &   26.0 &   0.09 &   $-$1.38 &    ...  &    ...  &   27.0  &   74.9  &   70.0  &   57.0  &   45.4  &    ...  &   87.1\tablenotemark{b} &   40.2  \\
 3886.28 &   26.0 &   0.05 &   $-$1.08 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 3887.05 &   26.0 &   0.91 &   $-$1.14 &    ...  &   93.2  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 3895.66 &   26.0 &   0.11 &   $-$1.67 &    ...  &    ...  &   18.0  &   86.8\tablenotemark{b} &   41.8  &   36.2  &    ...  &    ...  &   61.3  &   38.7  \\
 3899.71 &   26.0 &   0.09 &   $-$1.53 &    ...  &   97.4  &   30.0  &   65.8  &   53.4  &   44.7  &    ...  &    ...  &   69.8  &   38.8  \\
 3920.26 &   26.0 &   0.12 &   $-$1.75 &    ...  &    ...  &   15.6  &   42.8  &   44.3  &   46.2  &    ...  &    ...  &   62.2  &   19.9  \\
 3922.91 &   26.0 &   0.05 &   $-$1.65 &  134.0  &    ...  &   21.0  &   62.7  &   56.8  &   45.6  &   41.2  &    ...  &   62.5  &   28.8  \\
 4005.24 &   26.0 &   1.56 &   $-$0.61 &  108.0  &    ...  &   14.2  &   27.0  &   34.8  &   31.5  &    ...  &    ...  &   54.9  &   14.4  \\
 4045.81 &   26.0 &   1.48 &    0.28 &  133.0  &    ...  &   43.0  &   70.9  &   76.9  &   67.6  &   61.5  &   48.7  &   87.3  &   57.0  \\
 4063.59 &   26.0 &   1.56 &    0.07 &  133.0  &    ...  &   31.2  &   71.4  &   70.8  &   65.8  &   49.3  &   37.6  &   76.1  &   45.2  \\
 4071.74 &   26.0 &   1.61 &   $-$0.02 &  116.5  &    ...  &   27.2  &   52.8  &   52.7  &   63.9  &   41.3  &   33.7  &   69.8  &   40.1  \\
 4076.63 &   26.0 &   3.21 &   $-$0.37 &    ...  &    ...  &    ...  &    ...  &   11.2  &    ...  &    ...  &    ...  &   12.5  &    ...  \\
 4132.06 &   26.0 &   1.61 &   $-$0.67 &  102.2  &    ...  &    ...  &    ...  &   33.7  &   30.4  &    ...  &   13.4  &   48.1  &   19.0  \\
 4134.68 &   26.0 &   2.83 &   $-$0.49 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4143.87 &   26.0 &   1.56 &   $-$0.46 &  103.5  &    ...  &   13.9  &   33.8  &   38.4  &   44.5  &   44.9  &   15.9  &   55.3  &   19.7  \\
 4147.67 &   26.0 &   1.48 &   $-$2.10 &   39.7  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4156.80 &   26.0 &   2.83 &   $-$0.61 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4181.76 &   26.0 &   2.83 &   $-$0.18 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   13.1  &    ...  \\
 4187.04 &   26.0 &   2.45 &   $-$0.55 &   56.3  &    ...  &    ...  &   22.3  &    ...  &    ...  &    ...  &    ...  &   13.4  &    ...  \\
 4187.80 &   26.0 &   2.42 &   $-$0.55 &    ...  &    ...  &    ...  &    ...  &   19.0  &    ...  &    ...  &    ...  &   12.1  &    ...  \\
 4191.43 &   26.0 &   2.47 &   $-$0.73 &   34.1  &   74.1\tablenotemark{b} &    ...  &    ...  &    8.1 &    ...  &    ...  &    ...  &   15.1  &    6.2 \\
 4199.10 &   26.0 &   3.05 &    0.25 &    ...  &    ...  &    ...  &    ...  &   11.2  &    ...  &    ...  &    ...  &   23.5  &    ...  \\
 4202.03 &   26.0 &   1.48 &   $-$0.70 &    ...  &    ...  &   12.0  &   24.0  &   42.5  &   32.0  &    ...  &   17.0  &   57.8  &   16.6  \\
 4222.21 &   26.0 &   2.45 &   $-$0.97 &    ...  &   38.8  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   14.1  &    ...  \\
 4227.43 &   26.0 &   3.33 &    0.23 &   39.0  &   81.6\tablenotemark{b} &    ...  &    ...  &    ...  &   15.8  &    ...  &    ...  &   20.9  &    ...  \\
 4233.60 &   26.0 &   2.48 &   $-$0.60 &   41.0  &   48.8  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   15.1  &    ...  \\
 4250.12 &   26.0 &   2.47 &   $-$0.40 &   71.9  &    ...  &    ...  &    ...  &   13.2  &   17.2  &    ...  &    ...  &   23.2  &    ...  \\
 4260.47 &   26.0 &   2.40 &   $-$0.02 &   79.6  &   79.1  &    6.6  &   29.9  &   29.9  &    ...  &    ...  &    8.8  &   49.1  &   14.6  \\
 4271.15 &   26.0 &   2.45 &   $-$0.35 &    ...  &    ...  &    ...  &    ...  &   16.4  &   17.3  &    ...  &    4.0 &   24.6  &    5.6 \\
 4271.76 &   26.0 &   1.48 &   $-$0.16 &    ...  &    ...  &   33.7  &   62.1  &   63.3  &   57.7  &   46.2  &   31.7  &   73.6  &   41.7  \\
 4282.40 &   26.0 &   2.17 &   $-$0.82 &   52.8  &   61.9  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   13.9  &    ...  \\
 4325.76 &   26.0 &   1.61 &   $-$0.01 &    ...  &    ...  &   27.0  &   58.5  &   55.8  &   51.7  &   45.5  &   33.2  &   66.7  &   37.2  \\
 4383.55 &   26.0 &   1.48 &    0.20 &  138.0  &    ...  &   46.5  &   72.4  &   79.8  &   79.7  &   66.7  &   48.2  &   85.9  &   51.6  \\
 4404.75 &   26.0 &   1.56 &   $-$0.14 &  123.0  &    ...  &   28.2  &   56.8  &   69.3  &   55.1  &    ...  &   30.5  &   76.4  &   38.8  \\
 4415.12 &   26.0 &   1.61 &   $-$0.61 &  110.5  &    ...  &    ...  &   36.2  &   33.0  &   34.7  &   29.3  &   13.4  &   50.5  &   17.2  \\
 4442.34 &   26.0 &   2.20 &   $-$1.25 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   12.6  &    ...  \\
 4447.72 &   26.0 &   2.22 &   $-$1.34 &   40.8  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4461.65 &   26.0 &   0.09 &   $-$3.20 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   10.1  &    ...  \\
 4466.55 &   26.0 &   2.83 &   $-$0.60 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   11.4  &    ...  \\
 4489.74 &   26.0 &   0.12 &   $-$3.97 &   35.4  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4494.56 &   26.0 &   2.20 &   $-$1.14 &   46.7  &   47.3  &    ...  &    ...  &    ...  &    8.7 &   17.0\tablenotemark{b} &    ...  &    ...  &    ...  \\
 4528.61 &   26.0 &   2.18 &   $-$0.82 &   68.0  &   63.0  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   13.4  &    ...  \\
 4531.15 &   26.0 &   1.48 &   $-$2.15 &   38.6  &   53.1  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4871.32 &   26.0 &   2.87 &   $-$0.36 &   44.8  &   62.5  &    ...  &   10.7 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4872.14 &   26.0 &   2.88 &   $-$0.57 &   23.7  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4891.49 &   26.0 &   2.85 &   $-$0.11 &   53.3  &   81.8\tablenotemark{b} &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   21.8  &    ...  \\
 4903.31 &   26.0 &   2.88 &   $-$0.93 &    ...  &   23.4  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4918.99 &   26.0 &   2.87 &   $-$0.34 &   41.0  &   52.8  &    ...  &    ...  &    ...  &   15.8  &    ...  &    ...  &   12.2  &    ...  \\
 4920.50 &   26.0 &   2.83 &    0.07 &   66.9  &    ...  &    ...  &    ...  &   20.8  &   20.0  &    ...  &    ...  &   27.2  &    6.9 \\
 4939.69 &   26.0 &   0.86 &   $-$3.34 &   24.6  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4994.13 &   26.0 &   0.92 &   $-$3.08 &   32.0  &   22.7  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5006.12 &   26.0 &   2.83 &   $-$0.62 &   34.2  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5041.76 &   26.0 &   1.49 &   $-$2.20 &   46.5  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5051.64 &   26.0 &   0.92 &   $-$2.80 &   46.0  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5083.34 &   26.0 &   0.96 &   $-$2.96 &   34.9  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5123.72 &   26.0 &   1.01 &   $-$3.07 &   32.8  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5127.36 &   26.0 &   0.92 &   $-$3.31 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5150.84 &   26.0 &   0.99 &   $-$3.04 &   29.4  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5166.28 &   26.0 &   0.00 &   $-$4.20 &   36.5  &   25.5  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   15.2\tablenotemark{b} &    ...  \\
 5171.60 &   26.0 &   1.49 &   $-$1.79 &   66.5  &   51.8  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   10.4  &    ...  \\
 5191.46 &   26.0 &   3.04 &   $-$0.55 &    ...  &   44.7  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5192.34 &   26.0 &   3.00 &   $-$0.42 &    ...  &   42.8  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5194.94 &   26.0 &   1.56 &   $-$2.09 &   39.0  &   43.5  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5216.27 &   26.0 &   1.61 &   $-$2.15 &   35.8  &   36.1  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5232.94 &   26.0 &   2.94 &   $-$0.06 &   48.0  &   67.9  &    ...  &    ...  &   15.4  &   18.2  &    ...  &    ...  &   23.3  &    ...  \\
 5266.56 &   26.0 &   3.00 &   $-$0.39 &   28.2  &   43.8  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5269.54 &   26.0 &   0.86 &   $-$1.32 &    ...  &   99.0  &    ...  &    ...  &   29.0  &   33.6  &    ...  &   12.6  &   54.0  &   18.6  \\
 5281.79 &   26.0 &   3.04 &   $-$0.83 &    ...  &   18.5  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5283.62 &   26.0 &   3.24 &   $-$0.52 &   25.9  &   27.3  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5324.18 &   26.0 &   3.21 &   $-$0.24 &   26.3  &   43.2  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   15.6  &    ...  \\
 5328.04 &   26.0 &   0.92 &   $-$1.47 &  131.0  &   88.2  &    ...  &    ...  &   32.5  &   29.5  &    ...  &    8.8  &   41.5  &   12.5  \\
 5328.53 &   26.0 &   1.56 &   $-$1.85 &   65.9  &   41.2  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5371.49 &   26.0 &   0.96 &   $-$1.65 &  112.5  &   90.2  &    ...  &   25.0  &   25.8  &   24.0  &    ...  &    ...  &   40.2  &    8.4  \\
 5397.13 &   26.0 &   0.92 &   $-$1.99 &  108.0  &   66.3  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   20.5  &    ...  \\
 5405.78 &   26.0 &   0.99 &   $-$1.84 &   97.7  &   70.9  &    ...  &    ...  &   16.2  &    ...  &    ...  &    ...  &   26.8  &    6.8 \\
 5429.70 &   26.0 &   0.96 &   $-$1.88 &  102.8  &   78.1  &    ...  &    ...  &   15.8  &    ...  &    ...  &    ...  &   21.2  &    5.3 \\
 5434.52 &   26.0 &   1.01 &   $-$2.12 &   79.2  &   71.1  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   15.5  &    ...  \\
 5446.92 &   26.0 &   0.99 &   $-$1.91 &  105.0  &   75.5  &    ...  &    ...  &    9.6 &    ...  &    ...  &    7.4\tablenotemark{b} &   14.9  &    ...  \\
 5455.61 &   26.0 &   1.01 &   $-$2.09 &   86.3  &    ...  &    ...  &    ...  &    ...  &   88.4\tablenotemark{b} &    ...  &    ...  &   21.0  &    ...  \\
 5497.52 &   26.0 &   1.01 &   $-$2.85 &   36.8  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   11.8\tablenotemark{b} &    ...  &    ...  \\
 5501.47 &   26.0 &   0.96 &   $-$3.05 &   26.9  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5506.78 &   26.0 &   0.99 &   $-$2.80 &   46.2  &   25.9  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5572.84 &   26.0 &   3.40 &   $-$0.31 &   19.2  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5586.76 &   26.0 &   3.37 &   $-$0.14 &   27.5  &   37.6  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5615.64 &   26.0 &   3.33 &   $-$0.14 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 6136.62 &   26.0 &   2.45 &   $-$1.40 &   29.3  &   23.0  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 6137.69 &   26.0 &   2.59 &   $-$1.40 &    ...  &   17.1  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 6191.56 &   26.0 &   2.43 &   $-$1.42 &    ...  &   23.2  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 6230.72 &   26.0 &   2.56 &   $-$1.28 &   28.2  &   28.4  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 6252.56 &   26.0 &   2.40 &   $-$1.69 &   16.5  &   18.8  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 6393.60 &   26.0 &   2.43 &   $-$1.58 &    ...  &   23.5  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 6494.98 &   26.0 &   2.40 &   $-$1.27 &   47.0  &   59.0  &    ...  &    ...  &   23.4\tablenotemark{b} &    ...  &    ...  &   12.8\tablenotemark{b} &    ...  &    ...  \\
 4178.86 &   26.1 &   2.58 &   $-$2.50 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4233.17 &   26.1 &   2.58 &   $-$1.90 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   12.4  &    ...  \\
 4508.29 &   26.1 &   2.86 &   $-$2.25 &    ...  &   21.3  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4520.22 &   26.1 &   2.81 &   $-$2.60 &   19.6  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4522.63 &   26.1 &   2.84 &   $-$2.03 &   40.2  &   56.2  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5197.58 &   26.1 &   3.23 &   $-$2.23 &    ...  &   18.2  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5234.63 &   26.1 &   3.22 &   $-$2.15 &   19.5  &   13.1  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 3845.46 &   27.0 &   0.92 &    0.01 &   89.8  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   16.1  &    ...  \\
 3995.30 &   27.0 &   0.92 &   $-$0.22 &   54.7  &   48.8  &    ...  &    ...  &    6.8  &    ...  &    ...  &    ...  &   12.5  &    ...  \\
 4118.77 &   27.0 &   1.05 &   $-$0.49 &   46.4  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4121.31 &   27.0 &   0.92 &   $-$0.32 &   60.8  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 3807.14 &   28.0 &   0.42 &   $-$1.18 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   35.5  &    ...  \\
 3858.29 &   28.0 &   0.42 &   $-$0.97 &    ...  &    ...  &   15.0  &    ...  &   30.5  &   22.8  &    ...  &    ...  &   40.5  &    ...  \\
 5476.90 &   28.0 &   1.83 &   $-$0.89 &   37.8  &   45.6  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4077.71 &   38.1 &   0.00 &    0.16 &  120.0  &  121.0  &    ...  &   59.5  &   74.0  &   26.1  &   51.8  &    ...  &   54.1  &   29.8  \\
 4215.52 &   38.1 &   0.00 &   $-$0.16 &  107.0  &    ...  &    ...  &   30.4  &   45.3  &   19.9  &    ...  &    ...  &   36.5  &   15.1  \\
 4554.03 &   56.1 &   0.00 &    0.16 &   73.8  &  168.5  &    ...  &    9.1  &   22.7  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4934.08 &   56.1 &   0.00 &   $-$0.15 &   61.6  &  187.0  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 6141.73 &   56.1 &   0.70 &   $-$0.08 &   33.3  &  110.5  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 6496.91 &   56.1 &   0.60 &   $-$0.38 &    ...  &  116.0  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
\enddata                                                                                                                
\tablenotetext{a}{$S/N$ per $\sim$0.17\,{\AA}~pixel at 4500\,{\AA}}                                                      
\tablenotetext{b}{These lines produce discrepant abundances and are not included in the results reported in Paper II}   
\end{deluxetable}                                                                                                       
\end{center}                                                                                                          



==> tab5.tex <==
\begin{center}                                                                                                          
\begin{deluxetable}{cccrrrrrrrrrrr}                                                                                     
\tabletypesize{\tiny}                                                                                                   
\tablecolumns{14}                                                                                                       
\tablewidth{0pt}                                                                                                        
\rotate                                                                                                                 
\tablecaption{\label{Tab:table5} ATOMIC DATA AND EQUIVALENT WIDTHS (m{\AA}) FOR PROGRAM STARS}                        
\tablehead{                                                                                                             
\colhead{Wavelength} & {Species} & {$\chi$} & {log$gf$} & {HE~1142} & {HE~1201} & {HE~1204} & {HE~1207} & {HE~1320} & {HE~1346} & {HE~1402} & {HE~1506} & {HE~2020} & {HE~2032} \\
{(\AA)}   & &{($\rm eV$)} &                             & {--1422}  & {--1512}  & {--0744}  & {--3108}  & {--2952}  & {--0427}  & {--0523}  & {--0113}  & {--5228}  & {--5633} \\
{(1)} & {(2)} & {(3)} & {(4)}                           & {(5)}     & {(6)}     & {(7)}     & {(8)}     & {(9)}     & {(10)}    & {(11)}    & {(12)}    &  {(13)}   & {(14)}
}                                                                                                                       
\startdata                                                                                                              
$S/N$\tablenotemark{a}  &  &  &  &    62 &    219 &     27 &     66 &     61 &    206 &     77 &     64 &     37 &     56 \\
W(min)\,(m{\AA})  &  &  &  &    15 &      5 &     16 &     10 &     10 &      5 &      8 &      5 &     13 &     10 \\\\
 5889.95 &   11.0 &   0.00 &    0.11 &   87.9  &   17.7  &   67.8  &  156.0  &   79.5  &   19.8  &   29.7  &  185.0  &    ...  &   23.5  \\
 5895.92 &   11.0 &   0.00 &   $-$0.19 &   53.7  &    8.5  &    ...  &  105.0  &   55.8  &   13.7  &   25.9  &  152.0  &    ...  &    9.9  \\
 3829.36 &   12.0 &   2.71 &   $-$0.21 &  139.5  &   60.7  &    ...  &  101.8  &  100.7  &    ...  &   86.7  &  138.0  &   85.5  &   59.6  \\
 3832.30 &   12.0 &   2.71 &    0.15 &    ...  &    ...  &    ...  &  128.5  &  123.0  &    ...  &    ...  &    ...  &  116.5  &    ...  \\
 3838.29 &   12.0 &   2.72 &    0.41 &    ...  &    ...  &    ...  &  143.0  &  136.5  &    ...  &    ...  &    ...  &  121.5  &    ...  \\
 4571.10 &   12.0 &   0.00 &   $-$5.39 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5172.68 &   12.0 &   2.71 &   $-$0.38 &  165.5  &   61.0  &    ...  &  103.5  &  109.0  &   64.6  &   79.8  &  155.0  &  111.5  &   53.8  \\
 5183.60 &   12.0 &   2.72 &   $-$0.16 &  179.0  &   75.7  &  102.5  &  125.0  &  121.0  &   77.5  &   88.2  &  174.0  &  106.0  &   72.8  \\
 5528.41 &   12.0 &   4.34 &   $-$0.34 &   25.8  &    7.8  &    ...  &   16.0  &    ...  &    4.9  &    ...  &   44.7  &   17.6  &    ...  \\
 3944.01 &   13.0 &   0.00 &   $-$0.64 &   56.1  &    ...  &    ...  &   65.7  &   63.1  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 3961.52 &   13.0 &   0.01 &   $-$0.34 &   69.2  &   19.4  &    ...  &   58.6  &   52.7  &    ...  &   23.8  &   81.0  &    ...  &   17.0  \\
 3905.52 &   14.0 &   1.91 &   $-$1.09 &   96.4  &   65.8  &   56.8  &  116.5  &  109.5  &    ...  &   54.5  &    ...  &   72.7  &   45.7  \\
 4226.73 &   20.0 &   0.00 &    0.24 &  163.0  &   69.4  &  122.0  &  115.0  &  106.5  &   73.3  &   82.2  &  131.0  &   97.4  &   82.3  \\
 4283.01 &   20.0 &   1.89 &   $-$0.22 &   14.6  &    ...  &    ...  &   22.5  &    ...  &    ...  &    ...  &    ...  &   13.8  &    ...  \\
 4318.65 &   20.0 &   1.90 &   $-$0.21 &    ...  &    ...  &    ...  &   19.7  &    ...  &    3.0  &    ...  &    ...  &    ...  &    ...  \\
 4435.68 &   20.0 &   1.89 &   $-$0.52 &    ...  &    ...  &    ...  &    8.7  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4454.78 &   20.0 &   1.90 &    0.26 &    ...  &    7.2  &   30.4  &   32.5  &   24.2  &    9.6  &   13.2  &    ...  &   23.1  &    ...  \\
 5588.75 &   20.0 &   2.52 &    0.21 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    7.3  &    ...  &    ...  \\
 5857.45 &   20.0 &   2.93 &    0.23 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 6122.22 &   20.0 &   1.89 &   $-$0.32 &    ...  &    ...  &    ...  &   15.8  &    ...  &    ...  &    ...  &    9.3  &    ...  &    ...  \\
 6162.17 &   20.0 &   1.90 &   $-$0.09 &    ...  &    ...  &    ...  &   17.0  &   14.6  &    4.4  &    ...  &   14.7  &    ...  &    ...  \\
 6439.08 &   20.0 &   2.52 &    0.47 &    ...  &    ...  &    ...  &   10.4  &    9.2  &    3.3  &    ...  &    8.0  &   22.6  &    ...  \\
 4246.82 &   21.1 &   0.31 &    0.24 &   76.6  &    7.1  &   21.2  &   49.5  &   47.8  &    8.2  &   20.0  &    ...  &   38.2  &    ...  \\
 4314.08 &   21.1 &   0.62 &   $-$0.10 &   38.5  &    ...  &    ...  &   20.8  &   20.2  &    ...  &    9.4  &    ...  &    ...  &    ...  \\
 3998.64 &   22.0 &   0.05 &   $-$0.06 &    ...  &    ...  &    ...  &   14.7  &    ...  &    ...  &    ...  &   30.3  &    ...  &    ...  \\
 4533.24 &   22.0 &   0.85 &    0.48 &    ...  &    ...  &    ...  &    ...  &   10.5  &    2.6  &    ...  &    ...  &    ...  &    ...  \\
 4981.73 &   22.0 &   0.84 &    0.50 &    ...  &    ...  &    ...  &   12.5  &   11.1  &    ...  &    ...  &   16.3  &    ...  &    ...  \\
 4991.07 &   22.0 &   0.84 &    0.38 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   18.7  &    ...  &    ...  \\
 4999.50 &   22.0 &   0.83 &    0.25 &    ...  &    ...  &    ...  &    ...  &    9.2  &    ...  &    ...  &   12.0  &    ...  &    ...  \\
 5192.97 &   22.0 &   0.02 &   $-$1.01 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 3759.30 &   22.1 &   0.61 &    0.27 &    ...  &   42.8  &   65.8 &   93.6  &  102.5  &    ...  &   75.6  &  124.0  &   78.2  &   67.2  \\
 3761.32 &   22.1 &   0.57 &    0.17 &    ...  &   38.4  &   64.7  &   96.8  &   83.8  &    ...  &    ...  &  106.0  &   71.2  &   47.9  \\
 3913.47 &   22.1 &   1.12 &   $-$0.41 &  118.0  &    7.2  &    ...  &   55.3  &   53.4  &    ...  &   25.4  &   74.0  &    ...  &   19.9  \\
 4012.39 &   22.1 &   0.57 &   $-$1.75 &   40.6  &    ...  &    ...  &   22.1  &   14.8  &    ...  &    ...  &   47.3  &   63.6\tablenotemark{b} &    ...  \\
 4028.34 &   22.1 &   1.89 &   $-$0.99 &   12.9  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   17.0  &    ...  &    ...  \\
 4290.22 &   22.1 &   1.16 &   $-$0.93 &   58.7  &    ...  &    ...  &   28.4  &   30.6  &    3.5  &    9.6  &    ...  &   24.2  &    ...  \\
 4300.05 &   22.1 &   1.18 &   $-$0.49 &   93.5  &    ...  &   31.0  &   45.2  &   44.2  &    8.2  &   18.5  &    ...  &   31.8  &    9.9  \\
 4395.03 &   22.1 &   1.08 &   $-$0.51 &  108.5  &    8.2  &    ...  &   53.9  &   54.0  &    8.7  &   29.0  &    ...  &    ...  &    ...  \\
 4399.77 &   22.1 &   1.24 &   $-$1.22 &   34.8  &    ...  &    ...  &   18.8  &   12.9  &    ...  &    ...  &    ...  &    ...  &    9.9 \\
 4417.72 &   22.1 &   1.16 &   $-$1.23 &   34.0  &    ...  &    ...  &   14.0  &   13.9  &    ...  &   10.2  &    ...  &    ...  &    ...  \\
 4443.79 &   22.1 &   1.08 &   $-$0.70 &   91.7  &    ...  &   28.2  &   42.8  &   44.1  &    7.6  &   21.8  &   65.5  &   28.1  &    ...  \\
 4450.48 &   22.1 &   1.08 &   $-$1.51 &   30.6  &    ...  &    ...  &   14.5  &   13.2  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4464.45 &   22.1 &   1.16 &   $-$1.81 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4468.51 &   22.1 &   1.13 &   $-$0.60 &   97.5  &    ...  &   38.3  &   43.2  &   47.1  &    9.3  &   21.7  &   72.5  &   28.3  &    ...  \\
 4501.27 &   22.1 &   1.12 &   $-$0.76 &   73.8  &    ...  &   28.2  &   41.8  &   43.6  &    8.2  &   19.5  &   73.0  &   12.6\tablenotemark{b} &    ...  \\
 4533.97 &   22.1 &   1.24 &   $-$0.54 &   87.3  &    5.4  &   33.4  &   43.3  &   40.2  &    6.9  &   16.5  &    ...  &   30.8  &    ...  \\
 4563.76 &   22.1 &   1.22 &   $-$0.79 &   62.8  &    ...  &   27.7  &   31.9  &   32.5  &    4.9  &   18.6  &    ...  &   32.9  &    ...  \\
 4571.97 &   22.1 &   1.57 &   $-$0.23 &    ...  &    4.9  &    ...  &   35.3  &   28.8  &    5.7  &   22.1  &    ...  &   25.0  &   13.0  \\
 5185.91 &   22.1 &   1.89 &   $-$1.37 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    6.0  &    ...  &    ...  \\
 5188.68 &   22.1 &   1.58 &   $-$1.05 &   46.7  &    ...  &    ...  &    ...  &   11.1  &    ...  &    ...  &   23.0  &    ...  &    ...  \\
 5226.54 &   22.1 &   1.57 &   $-$1.23 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   15.3  &   34.6\tablenotemark{b} &    ...  \\
 4254.33 &   24.0 &   0.00 &   $-$0.11 &   60.1  &    8.9  &   26.6  &   63.5  &   43.6  &   10.7  &   20.0  &   64.5  &   26.5  &    ...  \\
 4274.80 &   24.0 &   0.00 &   $-$0.23 &   54.5  &    7.6  &    ...  &   58.0  &   44.2  &    7.7  &   13.9  &    ...  &    ...  &    ...  \\
 4289.72 &   24.0 &   0.00 &   $-$0.36 &    ...  &    ...  &   29.4  &   56.0  &   30.5  &    7.2  &   12.4  &    ...  &   22.1  &    ...  \\
 5206.04 &   24.0 &   0.94 &    0.02 &    ...  &    ...  &    ...  &   35.0  &   21.0  &    ...  &    ...  &   33.7  &    ...  &    ...  \\
 5208.42 &   24.0 &   0.94 &    0.16 &    ...  &    ...  &   45.3  &   57.2  &    ...  &    3.2  &    ...  &   39.7  &    ...  &    ...  \\
 4030.75 &   25.0 &   0.00 &   $-$0.48 &   24.6  &    6.4  &    ...  &   74.1  &   27.2  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4033.06 &   25.0 &   0.00 &   $-$0.62 &   17.9  &    4.6  &    ...  &   61.2  &   32.5  &    ...  &    ...  &   68.5  &    ...  &    ...  \\
 4034.48 &   25.0 &   0.00 &   $-$0.81 &   23.5  &    6.9  &    ...  &   52.2  &   17.4  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 3743.36 &   26.0 &   0.99 &   $-$0.79 &    ...  &   38.8  &    ...  &    ...  &   77.8  &    ...  &   41.5  &   92.5  &    ...  &    ...  \\
 3758.23 &   26.0 &   0.96 &   $-$0.03 &    ...  &   71.3  &    ...  &  129.5  &  110.5  &    ...  &   60.8  &  114.0  &    ...  &    ...  \\
 3763.79 &   26.0 &   0.99 &   $-$0.24 &    ...  &   64.4  &    ...  &  109.5  &   95.0  &    ...  &   52.9  &   98.5  &    ...  &    ...  \\
 3765.54 &   26.0 &   3.24 &    0.48 &    ...  &    ...  &    ...  &   41.9 &    ...  &    ...  &    ...  &   32.3  &    ...  &    ...  \\
 3767.19 &   26.0 &   1.01 &   $-$0.39 &    ...  &   58.7  &    ...  &  112.5  &   82.8  &    ...  &    ...  &    ...  &   63.7  &    ...  \\
 3786.68 &   26.0 &   1.01 &   $-$2.23 &    ...  &    ...  &    ...  &   53.0  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 3787.88 &   26.0 &   1.01 &   $-$0.86 &    ...  &   30.8  &    ...  &   97.6  &   76.8  &    ...  &   35.7  &    ...  &   46.2  &    ...  \\
 3805.34 &   26.0 &   3.30 &    0.31 &    ...  &    8.2  &    ...  &   44.5  &   23.3  &    ...  &    ...  &   33.3  &    ...  &    ...  \\
 3815.84 &   26.0 &   1.48 &    0.24 &  133.5  &   64.0  &   96.5  &  122.0  &   95.9  &    ...  &   62.5  &  102.0  &   82.4  &   59.5  \\
 3820.43 &   26.0 &   0.86 &    0.12 &  176.5  &   86.0  &    ...  &  161.5  &  119.0  &    ...  &   80.1  &  124.0  &    ...  &   67.9  \\
 3824.44 &   26.0 &   0.00 &   $-$1.36 &  116.0  &   70.3  &    ...  &  137.5  &  104.5  &    ...  &   54.8  &  120.0  &   72.0  &   45.4  \\
 3825.88 &   26.0 &   0.91 &   $-$0.04 &  153.5  &   79.8  &  103.0  &  151.0  &  104.0  &    ...  &   72.0  &  126.0  &   87.6  &   56.2  \\
 3827.82 &   26.0 &   1.56 &    0.06 &  123.5  &   51.3  &    ...  &  113.5  &   82.5  &    ...  &   59.7  &   92.0  &   61.2  &   35.2  \\
 3840.44 &   26.0 &   0.99 &   $-$0.51 &  120.5  &   55.0  &   82.8  &  110.5  &   85.0  &    ...  &   55.9  &  103.0  &    ...  &    ...  \\
 3849.97 &   26.0 &   1.01 &   $-$0.97 &   91.5  &   38.4  &   58.4  &  102.2  &   75.3  &    ...  &   42.0  &   87.5  &    ...  &    ...  \\
 3850.82 &   26.0 &   0.99 &   $-$1.73 &    ...  &    9.5  &    ...  &   68.8  &   38.2  &    ...  &   18.6  &   59.3  &   29.5  &    ...  \\
 3856.37 &   26.0 &   0.05 &   $-$1.29 &  138.0  &   67.5  &   70.2  &  119.5  &  104.0  &    ...  &   59.1  &  105.0  &   81.2  &   50.7  \\
 3859.91 &   26.0 &   0.00 &   $-$0.71 &  180.0  &   94.3  &  118.5  &  160.0  &  121.5  &    ...  &   88.1  &  136.0  &  101.5  &   73.6  \\
 3865.52 &   26.0 &   1.01 &   $-$0.98 &   75.2  &   34.8  &    ...  &   97.3  &   71.5  &    ...  &   25.5  &   86.5  &   54.8  &    ...  \\
 3878.02 &   26.0 &   0.96 &   $-$0.91 &   80.3  &   39.4  &   38.8\tablenotemark{b} &   96.9  &   75.6  &    ...  &   41.8  &   92.0  &   58.8  &   23.7  \\
 3878.57 &   26.0 &   0.09 &   $-$1.38 &  129.5  &   60.0  &   90.1  &  158.0  &  108.0\tablenotemark{b} &    ...  &   58.7  &    ...  &   74.9  &   41.1  \\
 3886.28 &   26.0 &   0.05 &   $-$1.08 &    ...  &    ...  &    ...  &  138.5  &  103.5  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 3887.05 &   26.0 &   0.91 &   $-$1.14 &    ...  &    ...  &    ...  &    ...  &   72.6  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 3895.66 &   26.0 &   0.11 &   $-$1.67 &   80.1  &   46.6  &    ...  &  103.5  &   84.7  &    ...  &   38.0  &    ...  &   47.6  &   22.0  \\
 3899.71 &   26.0 &   0.09 &   $-$1.53 &   96.6  &   59.5  &   65.0  &  116.5  &   92.3  &    ...  &   48.0  &  102.0  &   60.5  &   27.2  \\
 3920.26 &   26.0 &   0.12 &   $-$1.75 &   92.2  &   42.9  &   43.2  &  101.0  &   85.3  &    ...  &   40.8  &    ...  &   46.2  &    ...  \\
 3922.91 &   26.0 &   0.05 &   $-$1.65 &   99.1  &   52.8  &   67.9  &  106.0  &   93.3  &    ...  &   48.6  &  110.0  &    ...  &    ...  \\
 4005.24 &   26.0 &   1.56 &   $-$0.61 &   69.2  &   26.0  &    ...  &   84.3  &   70.8  &    ...  &   25.3  &   75.0  &   52.1  &    ...  \\
 4045.81 &   26.0 &   1.48 &    0.28 &  161.5  &   67.1  &   96.2  &  132.0  &   95.2  &   60.8  &   65.8  &  108.0  &   81.9  &   72.3\tablenotemark{b} \\
 4063.59 &   26.0 &   1.56 &    0.07 &  131.0  &   55.3  &   86.7  &  112.5  &   76.6  &   48.3  &   55.5  &  106.0  &   78.8  &    ...  \\
 4071.74 &   26.0 &   1.61 &   $-$0.02 &  114.5  &   47.8  &   70.8  &  105.5  &   78.8  &   43.8  &   51.0  &   91.5  &   69.9  &   36.0  \\
 4076.63 &   26.0 &   3.21 &   $-$0.37 &    ...  &    ...  &    ...  &   28.2  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4132.06 &   26.0 &   1.61 &   $-$0.67 &   64.3  &   22.6  &   38.3  &   85.5  &   64.8  &   18.2  &   21.7  &   75.0  &   44.3  &    ...  \\
 4134.68 &   26.0 &   2.83 &   $-$0.49 &    ...  &    ...  &   21.6  &   25.8  &   13.9  &    ...  &    9.8  &    ...  &    ...  &    ...  \\
 4143.87 &   26.0 &   1.56 &   $-$0.46 &   76.3  &   28.5  &   65.8  &   92.1  &   64.5  &   23.8  &   29.5  &   76.0  &   52.2  &   22.9  \\
 4147.67 &   26.0 &   1.48 &   $-$2.10 &    ...  &    ...  &    ...  &   32.1  &    ...  &    ...  &    ...  &   18.3  &    ...  &    ...  \\
 4156.80 &   26.0 &   2.83 &   $-$0.61 &    ...  &    ...  &    ...  &   26.5  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4181.76 &   26.0 &   2.83 &   $-$0.18 &   16.0  &    ...  &    ...  &   42.9  &   19.8  &    ...  &    7.6 &   31.7  &    ...  &    ...  \\
 4187.04 &   26.0 &   2.45 &   $-$0.55 &   27.5  &    5.4  &    ...  &   55.2  &   24.8  &    4.6 &    ...  &   33.0  &   19.5  &    ...  \\
 4187.80 &   26.0 &   2.42 &   $-$0.55 &   24.5  &    5.7  &    ...  &   54.8  &   20.5  &    5.8  &    8.9  &    ...  &   25.0  &    ...  \\
 4191.43 &   26.0 &   2.47 &   $-$0.73 &   27.8  &    ...  &    ...  &   48.4  &   18.8  &    ...  &    ...  &   23.7  &    ...  &    ...  \\
 4199.10 &   26.0 &   3.05 &    0.25 &   34.2  &    6.2  &   17.7  &   55.8  &    ...  &    5.4  &   14.5  &    ...  &    ...  &    ...  \\
 4202.03 &   26.0 &   1.48 &   $-$0.70 &   74.8  &   26.8  &   41.3  &   92.2  &   63.5  &   23.5  &   31.9  &    ...  &   52.4  &   22.9  \\
 4222.21 &   26.0 &   2.45 &   $-$0.97 &    ...  &    ...  &    ...  &   38.8  &   16.9  &    ...  &    ...  &   20.7  &    ...  &    ...  \\
 4227.43 &   26.0 &   3.33 &    0.23 &    ...  &    ...  &    ...  &   44.5  &   16.5  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4233.60 &   26.0 &   2.48 &   $-$0.60 &   24.9  &    6.0  &    ...  &   49.6  &   20.7  &    4.3 &    ...  &   31.7  &    ...  &    ...  \\
 4250.12 &   26.0 &   2.47 &   $-$0.40 &   36.2  &    6.5  &   17.8  &   59.8  &   25.3  &    7.3  &    ...  &   39.3  &    ...  &    ...  \\
 4260.47 &   26.0 &   2.40 &   $-$0.02 &   60.5  &   17.5  &   46.4  &   82.8  &   52.0  &   18.0  &   25.9  &   68.0  &   42.7  &    ...  \\
 4271.15 &   26.0 &   2.45 &   $-$0.35 &   36.5  &    7.2  &   27.3  &   59.2  &   33.0  &    8.4  &   15.7  &    ...  &   30.9  &    ...  \\
 4271.76 &   26.0 &   1.48 &   $-$0.16 &  125.5  &   49.8  &    ...  &  107.5  &   81.3  &   43.3  &   54.7  &    ...  &   71.9  &   37.6  \\
 4282.40 &   26.0 &   2.17 &   $-$0.82 &   24.1  &    ...  &    ...  &   54.9  &   26.8  &    3.7 &    ...  &   35.7  &   15.4  &    ...  \\
 4325.76 &   26.0 &   1.61 &   $-$0.01 &  117.5  &   49.0  &   79.8  &  115.0  &   81.9  &   43.9  &   54.5  &    ...  &   64.9  &   40.1  \\
 4383.55 &   26.0 &   1.48 &    0.20 &  154.0  &   68.8  &   89.6  &  128.5  &   95.8  &   61.2  &   70.1  &  109.0  &   81.8  &   54.0  \\
 4404.75 &   26.0 &   1.56 &   $-$0.14 &  111.5  &   50.3  &   73.0  &  115.5  &   74.8  &   42.4  &   54.7  &   90.0  &   71.6  &   34.6  \\
 4415.12 &   26.0 &   1.61 &   $-$0.61 &   63.0  &   26.0  &   64.2  &    ...  &   57.9  &   20.1  &   27.1  &   80.5  &   41.0  &   10.9  \\
 4442.34 &   26.0 &   2.20 &   $-$1.25 &    ...  &    ...  &    ...  &   33.0  &   11.7  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4447.72 &   26.0 &   2.22 &   $-$1.34 &    ...  &    ...  &    ...  &   36.0  &    ...  &    ...  &    ...  &   21.0  &    ...  &    ...  \\
 4461.65 &   26.0 &   0.09 &   $-$3.20 &    ...  &    5.6  &   15.5 &   58.1  &   26.4  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4466.55 &   26.0 &   2.83 &   $-$0.60 &    ...  &    ...  &    ...  &   33.3  &    ...  &    ...  &    5.8 &    ...  &   31.5\tablenotemark{b} &    ...  \\
 4489.74 &   26.0 &   0.12 &   $-$3.97 &    ...  &    ...  &    ...  &   21.9  &    ...  &    ...  &    ...  &   15.3  &    ...  &    ...  \\
 4494.56 &   26.0 &   2.20 &   $-$1.14 &    ...  &    ...  &    ...  &   41.8  &   15.9  &    ...  &    ...  &   22.7  &    ...  &    ...  \\
 4528.61 &   26.0 &   2.18 &   $-$0.82 &   20.2  &    5.4  &   15.9 &   57.3  &   23.7  &    4.6 &    8.1  &    ...  &   15.1  &    ...  \\
 4531.15 &   26.0 &   1.48 &   $-$2.15 &    ...  &    ...  &    ...  &   31.0  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4871.32 &   26.0 &   2.87 &   $-$0.36 &    ...  &    ...  &    ...  &   46.0  &   18.3  &    ...  &    ...  &   23.3  &    ...  &    ...  \\
 4872.14 &   26.0 &   2.88 &   $-$0.57 &    ...  &    ...  &    ...  &   36.2  &   15.0  &    ...  &    ...  &   12.3  &   12.7 &    ...  \\
 4891.49 &   26.0 &   2.85 &   $-$0.11 &   27.1  &    5.4  &   29.4  &   54.3  &   20.5  &    ...  &    ...  &   32.7  &    ...  &    ...  \\
 4903.31 &   26.0 &   2.88 &   $-$0.93 &    ...  &    ...  &    ...  &   21.2  &    ...  &    ...  &    ...  &    7.3  &    ...  &    ...  \\
 4918.99 &   26.0 &   2.87 &   $-$0.34 &   20.6  &    ...  &    ...  &   43.2  &   17.6  &    3.9 &    ...  &   21.0  &    ...  &    ...  \\
 4920.50 &   26.0 &   2.83 &    0.07 &   29.0  &    8.7  &    ...  &   59.8  &   36.9  &    8.2  &    ...  &   43.0  &   19.5  &    ...  \\
 4939.69 &   26.0 &   0.86 &   $-$3.34 &    ...  &    ...  &    ...  &   16.2  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4994.13 &   26.0 &   0.92 &   $-$3.08 &    ...  &    ...  &    ...  &   23.1  &    ...  &    ...  &    ...  &   10.7  &    ...  &    ...  \\
 5006.12 &   26.0 &   2.83 &   $-$0.62 &    ...  &    ...  &    ...  &   29.4  &    ...  &    ...  &    ...  &   11.7  &    ...  &    ...  \\
 5041.76 &   26.0 &   1.49 &   $-$2.20 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   16.0  &    ...  &   21.0\tablenotemark{b} \\
 5051.64 &   26.0 &   0.92 &   $-$2.80 &    ...  &    ...  &   54.9\tablenotemark{b} &   48.5  &    ...  &    ...  &    ...  &   21.0  &    ...  &    ...  \\
 5083.34 &   26.0 &   0.96 &   $-$2.96 &    ...  &    ...  &    ...  &   29.3  &    ...  &    ...  &    ...  &   12.7  &    ...  &    ...  \\
 5123.72 &   26.0 &   1.01 &   $-$3.07 &    ...  &    ...  &    ...  &   29.5  &    ...  &    ...  &    ...  &    9.7  &    ...  &    ...  \\
 5127.36 &   26.0 &   0.92 &   $-$3.31 &    ...  &    ...  &    ...  &   25.2  &    ...  &    ...  &    ...  &    7.0  &    ...  &    ...  \\
 5150.84 &   26.0 &   0.99 &   $-$3.04 &    ...  &    ...  &    ...  &   23.2  &    ...  &    ...  &    ...  &    8.3  &    ...  &    ...  \\
 5166.28 &   26.0 &   0.00 &   $-$4.20 &    ...  &    ...  &    ...  &   20.0  &    ...  &    ...  &    ...  &   12.3  &    ...  &    ...  \\
 5171.60 &   26.0 &   1.49 &   $-$1.79 &    ...  &    ...  &    ...  &   63.8  &   21.6  &    4.1 &    ...  &   32.7  &    ...  &    ...  \\
 5191.46 &   26.0 &   3.04 &   $-$0.55 &    ...  &    ...  &    ...  &   31.2  &    ...  &    ...  &    ...  &   11.7  &    ...  &    ...  \\
 5192.34 &   26.0 &   3.00 &   $-$0.42 &    ...  &    ...  &    ...  &   26.6  &    ...  &    ...  &    ...  &   15.7  &    ...  &    ...  \\
 5194.94 &   26.0 &   1.56 &   $-$2.09 &    ...  &    ...  &    ...  &   37.8  &    ...  &    ...  &    ...  &   19.3  &    ...  &    ...  \\
 5216.27 &   26.0 &   1.61 &   $-$2.15 &    ...  &    ...  &    ...  &   21.5  &    ...  &    ...  &    ...  &   13.3  &    ...  &    ...  \\
 5232.94 &   26.0 &   2.94 &   $-$0.06 &   27.2  &    ...  &   21.4  &   54.9  &    ...  &    5.2  &    ...  &   28.0  &    ...  &    ...  \\
 5266.56 &   26.0 &   3.00 &   $-$0.39 &    ...  &    ...  &    ...  &   31.5  &    ...  &    ...  &    ...  &   17.0  &    ...  &    ...  \\
 5269.54 &   26.0 &   0.86 &   $-$1.32 &   57.7  &   31.6  &   56.2  &   88.9  &   84.2  &   25.0  &   24.9  &   97.0  &    ...  &    ...  \\
 5281.79 &   26.0 &   3.04 &   $-$0.83 &    ...  &    ...  &   43.6\tablenotemark{b} &   27.5  &    ...  &    ...  &    ...  &    6.7  &    ...  &    ...  \\
 5283.62 &   26.0 &   3.24 &   $-$0.52 &    ...  &    ...  &    ...  &   29.8  &    ...  &    ...  &    ...  &    7.7  &    ...  &    ...  \\
 5324.18 &   26.0 &   3.21 &   $-$0.24 &    ...  &    ...  &    ...  &   40.9  &    ...  &    ...  &    ...  &   17.3  &    ...  &    ...  \\
 5328.04 &   26.0 &   0.92 &   $-$1.47 &   48.8  &   24.0  &   48.0  &  112.5\tablenotemark{b} &   68.7  &   25.5  &    ...  &   88.5  &    ...  &    ...  \\
 5328.53 &   26.0 &   1.56 &   $-$1.85 &    ...  &    ...  &    ...  &   44.2  &   12.5  &    ...  &    ...  &   27.0  &    ...  &    ...  \\
 5371.49 &   26.0 &   0.96 &   $-$1.65 &   30.8  &   18.9  &    ...  &   95.4\tablenotemark{b} &   59.8  &   12.8  &    ...  &   77.0  &    ...  &    ...  \\
 5397.13 &   26.0 &   0.92 &   $-$1.99 &   31.5  &    8.5  &    ...  &   81.5\tablenotemark{b} &   44.3  &    5.1  &    ...  &   62.5  &    ...  &    ...  \\
 5405.78 &   26.0 &   0.99 &   $-$1.84 &   36.4  &   10.8  &    ...  &   75.2  &   45.5  &    6.2  &    ...  &   65.0  &    ...  &    ...  \\
 5429.70 &   26.0 &   0.96 &   $-$1.88 &    ...  &   10.9  &   26.9  &   95.2\tablenotemark{b} &   40.8  &    8.7  &    ...  &   66.5  &    ...  &    ...  \\
 5434.52 &   26.0 &   1.01 &   $-$2.12 &   31.4  &    7.6  &    ...  &   61.0  &    ...  &    ...  &    ...  &   47.3  &    ...  &    ...  \\
 5446.92 &   26.0 &   0.99 &   $-$1.91 &   27.0  &    7.7  &   38.5  &   85.3\tablenotemark{b} &   49.8  &    ...  &    ...  &   59.0  &    ...  &    ...  \\
 5455.61 &   26.0 &   1.01 &   $-$2.09 &    ...  &    4.8 &    ...  &   79.8\tablenotemark{b} &   37.8  &    ...  &    ...  &   49.7  &    ...  &    ...  \\
 5497.52 &   26.0 &   1.01 &   $-$2.85 &    ...  &    ...  &    ...  &   30.8  &   14.0  &    ...  &    ...  &   15.0  &    ...  &    ...  \\
 5501.47 &   26.0 &   0.96 &   $-$3.05 &    ...  &    ...  &    ...  &   37.8  &    ...  &    ...  &    ...  &   10.7  &    ...  &    ...  \\
 5506.78 &   26.0 &   0.99 &   $-$2.80 &    ...  &    ...  &    ...  &   38.3  &    ...  &    ...  &    ...  &   17.3  &    ...  &    ...  \\
 5572.84 &   26.0 &   3.40 &   $-$0.31 &    ...  &    ...  &    ...  &   24.0  &    ...  &    ...  &    ...  &    9.7  &    ...  &    ...  \\
 5586.76 &   26.0 &   3.37 &   $-$0.14 &    ...  &    ...  &    ...  &   29.4  &    ...  &    ...  &    ...  &   14.3  &    ...  &    ...  \\
 5615.64 &   26.0 &   3.33 &   $-$0.14 &   24.4  &    ...  &    ...  &   38.7  &   14.2  &    ...  &    ...  &   16.7  &    ...  &    ...  \\
 6136.62 &   26.0 &   2.45 &   $-$1.40 &    ...  &    ...  &    ...  &   35.1  &    ...  &    ...  &    ...  &    8.7  &    ...  &    ...  \\
 6137.69 &   26.0 &   2.59 &   $-$1.40 &    ...  &    ...  &    ...  &   23.8  &    ...  &    ...  &    ...  &    7.0  &    ...  &    ...  \\
 6191.56 &   26.0 &   2.43 &   $-$1.42 &    ...  &    ...  &    ...  &   20.7  &    ...  &    ...  &    ...  &    8.7  &    ...  &    ...  \\
 6230.72 &   26.0 &   2.56 &   $-$1.28 &    ...  &    ...  &    ...  &   24.1  &    ...  &    ...  &    ...  &   11.7  &    ...  &    ...  \\
 6252.56 &   26.0 &   2.40 &   $-$1.69 &    ...  &    ...  &    ...  &   18.2  &    ...  &    ...  &    ...  &    7.3  &    ...  &    ...  \\
 6393.60 &   26.0 &   2.43 &   $-$1.58 &    ...  &    ...  &    ...  &   30.2  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 6494.98 &   26.0 &   2.40 &   $-$1.27 &    ...  &    ...  &    ...  &   39.0  &    ...  &    ...  &    ...  &   13.0  &    ...  &    ...  \\
 4178.86 &   26.1 &   2.58 &   $-$2.50 &   22.2  &    ...  &    ...  &   19.9  &   13.9  &    ...  &    ...  &    ...  &   12.4 &    ...  \\
 4233.17 &   26.1 &   2.58 &   $-$1.90 &   57.8  &    ...  &    ...  &   49.0  &   16.1  &    ...  &    ...  &    ...  &   16.7  &    ...  \\
 4508.29 &   26.1 &   2.86 &   $-$2.25 &   32.8  &    ...  &    ...  &   20.8  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4520.22 &   26.1 &   2.81 &   $-$2.60 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4522.63 &   26.1 &   2.84 &   $-$2.03 &    ...  &    ...  &    ...  &   31.3  &    8.7 &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5197.58 &   26.1 &   3.23 &   $-$2.23 &    ...  &    ...  &    ...  &   26.2  &    ...  &    ...  &    ...  &    6.0  &    ...  &    ...  \\
 5234.63 &   26.1 &   3.22 &   $-$2.15 &    ...  &    ...  &   28.3  &   20.7  &    ...  &    ...  &    ...  &    5.3  &    ...  &    ...  \\
 3845.46 &   27.0 &   0.92 &    0.01 &    ...  &    ...  &    ...  &   31.0  &   28.7  &    ...  &    ...  &   55.3  &    ...  &    ...  \\
 3995.30 &   27.0 &   0.92 &   $-$0.22 &    ...  &    9.4  &    ...  &   30.9  &    ...  &    ...  &    ...  &   38.3  &   17.5  &    ...  \\
 4118.77 &   27.0 &   1.05 &   $-$0.49 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    7.9  &   31.7  &    ...  &    ...  \\
 4121.31 &   27.0 &   0.92 &   $-$0.32 &    ...  &    ...  &    ...  &   21.2  &   21.7  &    ...  &    ...  &   39.3  &    ...  &    ...  \\
 3807.14 &   28.0 &   0.42 &   $-$1.18 &    ...  &   17.2  &    ...  &   62.5  &   41.8  &    ...  &    ...  &   79.5  &    ...  &    ...  \\
 3858.29 &   28.0 &   0.42 &   $-$0.97 &   64.2  &   25.4  &   28.9  &   57.2  &   58.2  &    ...  &   21.2  &   84.0  &   32.7  &    ...  \\
 5476.90 &   28.0 &   1.83 &   $-$0.89 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   29.0  &    ...  &    ...  \\
 4077.71 &   38.1 &   0.00 &    0.16 &  165.5  &    ...  &   51.4  &   70.4  &   70.3  &   19.0  &   46.9  &   62.5  &    ...  &    ...  \\
 4215.52 &   38.1 &   0.00 &   $-$0.16 &  141.5  &    ...  &   40.7  &   68.9  &   56.5  &   12.4  &   28.5  &   58.3  &   43.0  &    ...  \\
 4554.03 &   56.1 &   0.00 &    0.16 &   84.3  &    ...  &    ...  &    ...  &   12.4  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4934.08 &   56.1 &   0.00 &   $-$0.15 &   72.2  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   17.7  &    ...  &    ...  \\
 6141.73 &   56.1 &   0.70 &   $-$0.08 &   33.5  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 6496.91 &   56.1 &   0.60 &   $-$0.38 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
\enddata                                                                                                                
\tablenotetext{a}{$S/N$ per $\sim$0.17\,{\AA}~pixel at 4500\,{\AA}}                                                      
\tablenotetext{b}{These lines produce discrepant abundances and are not included in the results reported in Paper II}   
\end{deluxetable}                                                                               

\end{center}                                                                                                          



==> tab6.tex <==
\begin{center}                                                                                                          
\begin{deluxetable}{cccrrrrrrrrrr}                                                                                      
\tabletypesize{\tiny}                                                                                                   
\tablecolumns{13}                                                                                                       
\tablewidth{0pt}                                                                                                        
\rotate                                                                                                                 
\tablecaption{\label{Tab:table6} ATOMIC DATA AND EQUIVALENT WIDTHS (m{\AA}) FOR PROGRAM STARS}                       
\tablehead{                                                                                                             
\colhead{Wavelength} & {Species} & {$\chi$} & {log$gf$} & {HE~2047} & {HE~2135} & {HE~2136} & {HE~2139} & {HE~2141} & {HE~2142} & {HE~2202} & {HE~2246} & {HE~2247} \\
{(\AA)}   & &{($\rm eV$)} &                             & {--5612}  & {--1924}  & {--6030}  & {--5432}  & {--0726}  & {--5656}  & {--4831}  & {--2410}  & {--7400} \\
{(1)} & {(2)} & {(3)} & {(4)}                           & {(5)}     & {(6)}     & {(7)}     & {(8)}     & {(9)}     & {(10)}    & {(11)}    & {(12)}    & {(13)}
}                                                                                                                       
\startdata                                                                                                              
$S/N$\tablenotemark{a}  &  &  &  &    63 &     75 &     31 &     86 &     44 &     48 &     37 &     61 &     23 \\
W(min)\,(m{\AA})  &  &  &  &    10 &      7 &     15 &      8 &     10 &     15 &     15 &      8 &     20 \\\\
 5889.95 &   11.0 &   0.00 &    0.11 &   44.2  &   17.6 &   38.7  &  146.0  &   45.2  &  187.0  &    ...  &  142.0  &    ...  \\
 5895.92 &   11.0 &   0.00 &   $-$0.19 &   22.2  &   36.2  &   24.9  &  130.0  &   26.5  &  166.5  &  192.5  &  120.0  &  170.5  \\
 3829.36 &   12.0 &   2.71 &   $-$0.21 &   68.7  &   57.5  &   70.6  &  136.0  &   88.3  &  166.5  &    ...  &   85.3  &    ...  \\
 3832.30 &   12.0 &   2.71 &    0.15 &    ...  &    ...  &  120.0  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 3838.29 &   12.0 &   2.72 &    0.41 &    ...  &    ...  &  119.0  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4571.10 &   12.0 &   0.00 &   $-$5.39 &    ...  &    ...  &    ...  &    ...  &    ...  &   43.5  &    ...  &    ...  &   58.0  \\
 5172.68 &   12.0 &   2.71 &   $-$0.38 &   78.0  &   52.0  &    ...  &  161.0  &   90.8  &    ...  &  131.0  &  102.4  &    ...  \\
 5183.60 &   12.0 &   2.72 &   $-$0.16 &   78.2  &   64.6  &  111.5  &    ...  &  105.0  &    ...  &  154.0  &   87.8  &  198.0  \\
 5528.41 &   12.0 &   4.34 &   $-$0.34 &    ...  &    ...  &   35.5  &   48.9  &   19.5  &   76.3  &    ...  &    ...  &   69.8  \\
 3944.01 &   13.0 &   0.00 &   $-$0.64 &    ...  &   11.1  &    ...  &    ...  &   26.0  &    ...  &    ...  &   25.7  &    ...  \\
 3961.52 &   13.0 &   0.01 &   $-$0.34 &   30.0  &   16.0  &   49.3  &   70.7  &   33.3  &  119.5  &    ...  &   23.2  &    ...  \\
 3905.52 &   14.0 &   1.91 &   $-$1.09 &   62.6  &   40.0  &  135.0  &    ...  &   68.2  &    ...  &    ...  &   64.1  &    ...  \\
 4226.73 &   20.0 &   0.00 &    0.24 &   70.4  &   69.8 &  120.0  &    ...  &  104.0  &    ...  &    ...  &   94.8  &    ...  \\
 4283.01 &   20.0 &   1.89 &   $-$0.22 &   11.3  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4318.65 &   20.0 &   1.90 &   $-$0.21 &    5.1  &    ...  &    ...  &    ...  &    8.6  &   41.2  &   28.7  &    ...  &   70.1  \\
 4435.68 &   20.0 &   1.89 &   $-$0.52 &    ...  &    ...  &    ...  &    ...  &    ...  &   30.9  &    ...  &    7.2  &   45.1  \\
 4454.78 &   20.0 &   1.90 &    0.26 &   11.9  &    ...  &   29.0  &    ...  &   12.3  &    ...  &    ...  &   19.5  &    ...  \\
 5588.75 &   20.0 &   2.52 &    0.21 &    ...  &    ...  &    ...  &    ...  &    ...  &   35.5  &   17.2  &    ...  &   50.4  \\
 5857.45 &   20.0 &   2.93 &    0.23 &    ...  &   11.9  &    ...  &    ...  &    ...  &   19.6  &   16.0  &    ...  &   27.9  \\
 6122.22 &   20.0 &   1.89 &   $-$0.32 &    ...  &    ...  &    ...  &    ...  &    ...  &   45.7  &   26.0  &    ...  &   52.3  \\
 6162.17 &   20.0 &   1.90 &   $-$0.09 &    ...  &    ...  &    ...  &    ...  &    ...  &   62.8  &   33.3  &    ...  &   61.0  \\
 6439.08 &   20.0 &   2.52 &    0.47 &    ...  &    ...  &    ...  &    ...  &    ...  &   44.2  &   23.6  &   13.2  &   51.4  \\
 4246.82 &   21.1 &   0.31 &    0.24 &   29.3  &    9.0  &    ...  &    ...  &   26.5  &    ...  &    ...  &   26.2  &    ...  \\
 4314.08 &   21.1 &   0.62 &   $-$0.10 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 3998.64 &   22.0 &   0.05 &   $-$0.06 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4533.24 &   22.0 &   0.85 &    0.48 &    ...  &    ...  &    ...  &    ...  &    ...  &   31.8  &   21.5  &    ...  &   51.0  \\
 4981.73 &   22.0 &   0.84 &    0.50 &    ...  &    ...  &    ...  &    ...  &    ...  &   42.1  &    ...  &    ...  &    ...  \\
 4991.07 &   22.0 &   0.84 &    0.38 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   17.6  &    ...  &    ...  \\
 4999.50 &   22.0 &   0.83 &    0.25 &    ...  &    ...  &    ...  &    ...  &    ...  &   40.2  &    ...  &    ...  &   35.3  \\
 5192.97 &   22.0 &   0.02 &   $-$1.01 &    ...  &    ...  &    ...  &    ...  &    ...  &   26.0  &    ...  &   28.2 &   32.7  \\
 3759.30 &   22.1 &   0.61 &    0.27 &   65.3  &   55.5  &    ...  &   55.8  &   74.0  &    ...  &    ...  &    ...  &    ...  \\
 3761.32 &   22.1 &   0.57 &    0.17 &   61.7  &   51.5  &    ...  &    ...  &   80.3  &  151.5  &   99.8  &    ...  &    ...  \\
 3913.47 &   22.1 &   1.12 &   $-$0.41 &   30.7  &   13.2  &    ...  &   18.3  &   32.0  &  111.5  &    ...  &   34.0  &    ...  \\
 4012.39 &   22.1 &   0.57 &   $-$1.75 &    ...  &    ...  &    ...  &    ...  &    ...  &   88.0  &    ...  &    ...  &    ...  \\
 4028.34 &   22.1 &   1.89 &   $-$0.99 &    ...  &    ...  &    ...  &   22.0\tablenotemark{b} &    ...  &   41.0  &    ...  &    ...  &    ...  \\
 4290.22 &   22.1 &   1.16 &   $-$0.93 &   16.3  &    ...  &   24.6  &    ...  &   16.7  &    ...  &    ...  &   11.8  &    ...  \\
 4300.05 &   22.1 &   1.18 &   $-$0.49 &   25.4  &    9.6  &   49.1  &    ...  &   32.1  &    ...  &    ...  &   26.8  &    ...  \\
 4395.03 &   22.1 &   1.08 &   $-$0.51 &   29.0  &    ...  &   44.2  &    ...  &   38.1  &    ...  &    ...  &   28.2  &    ...  \\
 4399.77 &   22.1 &   1.24 &   $-$1.22 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4417.72 &   22.1 &   1.16 &   $-$1.23 &    ...  &    ...  &    ...  &    ...  &   12.8  &    ...  &    ...  &    ...  &    ...  \\
 4443.79 &   22.1 &   1.08 &   $-$0.70 &   26.2  &    6.8  &   39.2  &   14.4  &   28.3  &   97.6  &   63.5  &   21.6  &  101.5  \\
 4450.48 &   22.1 &   1.08 &   $-$1.51 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4464.45 &   22.1 &   1.16 &   $-$1.81 &    ...  &    ...  &    ...  &    8.4\tablenotemark{b} &    ...  &    ...  &   32.7  &    ...  &   56.3  \\
 4468.51 &   22.1 &   1.13 &   $-$0.60 &   23.0  &   10.9  &   37.0  &   21.6  &   30.0  &   94.8  &   85.4  &    ...  &  100.5  \\
 4501.27 &   22.1 &   1.12 &   $-$0.76 &   23.0  &    ...  &   28.7  &   10.2  &    ...  &   92.3  &   59.6  &   17.8  &   95.8  \\
 4533.97 &   22.1 &   1.24 &   $-$0.54 &   23.0  &    ...  &   44.2  &    ...  &   26.5  &   98.2  &   80.6  &   22.3  &  106.5  \\
 4563.76 &   22.1 &   1.22 &   $-$0.79 &   16.5  &    ...  &   32.0  &    ...  &    ...  &   83.3  &   56.7  &    7.9  &   93.0  \\
 4571.97 &   22.1 &   1.57 &   $-$0.23 &   25.3  &    ...  &   28.6  &    ...  &   23.4  &   90.8  &   85.8  &   19.9  &   91.9  \\
 5185.91 &   22.1 &   1.89 &   $-$1.37 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   16.4  &    ...  &   28.2  \\
 5188.68 &   22.1 &   1.58 &   $-$1.05 &    ...  &    ...  &    ...  &    ...  &    ...  &   51.5  &   27.4  &    ...  &    ...  \\
 5226.54 &   22.1 &   1.57 &   $-$1.23 &    ...  &    ...  &    ...  &    ...  &    ...  &   62.2  &    ...  &    ...  &    ...  \\
 4254.33 &   24.0 &   0.00 &   $-$0.11 &   32.0  &    ...  &   21.4  &   41.2  &   31.1  &   98.5  &    ...  &   26.1  &  108.5  \\
 4274.80 &   24.0 &   0.00 &   $-$0.23 &   18.6  &    7.3  &   31.4  &    ...  &   31.2  &    ...  &    ...  &   15.1  &    ...  \\
 4289.72 &   24.0 &   0.00 &   $-$0.36 &    ...  &    ...  &   23.8  &    ...  &   25.0  &    ...  &    ...  &    ...  &    ...  \\
 5206.04 &   24.0 &   0.94 &    0.02 &    ...  &    ...  &    ...  &    ...  &   14.0  &   78.4  &   54.2  &    ...  &   86.8  \\
 5208.42 &   24.0 &   0.94 &    0.16 &   32.0  &    ...  &    ...  &    ...  &    ...  &   92.8  &   64.9  &    ...  &   98.2  \\
 4030.75 &   25.0 &   0.00 &   $-$0.48 &   13.1  &    8.1  &    ...  &    ...  &   15.9  &    ...  &    ...  &   19.2  &    ...  \\
 4033.06 &   25.0 &   0.00 &   $-$0.62 &   11.1  &    ...  &    ...  &    ...  &    ...  &  100.8  &    ...  &   13.2  &    ...  \\
 4034.48 &   25.0 &   0.00 &   $-$0.81 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 3743.36 &   26.0 &   0.99 &   $-$0.79 &    ...  &   36.9  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 3758.23 &   26.0 &   0.96 &   $-$0.03 &   70.1  &   64.3  &   84.2  &   69.3  &   87.9  &    ...  &    ...  &   85.0  &    ...  \\
 3763.79 &   26.0 &   0.99 &   $-$0.24 &    ...  &   55.7  &    ...  &   60.3  &   79.1  &    ...  &    ...  &    ...  &    ...  \\
 3765.54 &   26.0 &   3.24 &    0.48 &    ...  &    ...  &    ...  &    ...  &   22.7  &   75.8  &    ...  &    ...  &    ...  \\
 3767.19 &   26.0 &   1.01 &   $-$0.39 &   66.9  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   78.8  &    ...  \\
 3786.68 &   26.0 &   1.01 &   $-$2.23 &    ...  &    ...  &    ...  &    ...  &    ...  &   94.2  &   37.0  &    ...  &    ...  \\
 3787.88 &   26.0 &   1.01 &   $-$0.86 &   39.8  &   30.7  &   61.8  &   42.9  &    ...  &    ...  &   91.3  &   50.9  &  125.5  \\
 3805.34 &   26.0 &   3.30 &    0.31 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 3815.84 &   26.0 &   1.48 &    0.24 &   59.5  &   58.2  &   84.3  &    ...  &   88.2  &    ...  &    ...  &   79.4  &    ...  \\
 3820.43 &   26.0 &   0.86 &    0.12 &    ...  &   77.8  &    ...  &   71.8  &  106.5  &    ...  &    ...  &   93.8  &    ...  \\
 3824.44 &   26.0 &   0.00 &   $-$1.36 &   68.7  &   58.6  &   92.0  &   75.2\tablenotemark{b} &   75.8  &    ...  &    ...  &   79.8  &    ...  \\
 3825.88 &   26.0 &   0.91 &   $-$0.04 &   74.8  &   71.3  &   73.4\tablenotemark{b} &   60.9  &   83.7  &    ...  &    ...  &   81.3  &    ...  \\
 3827.82 &   26.0 &   1.56 &    0.06 &   53.5  &   54.2  &   58.2\tablenotemark{b} &   48.5  &   68.4  &    ...  &    ...  &   68.7  &    ...  \\
 3840.44 &   26.0 &   0.99 &   $-$0.51 &    ...  &    ...  &   56.5\tablenotemark{b} &   54.1  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 3849.97 &   26.0 &   1.01 &   $-$0.97 &   45.0  &   28.0  &   69.3  &   45.1  &   48.3  &    ...  &    ...  &   47.0  &    ...  \\
 3850.82 &   26.0 &   0.99 &   $-$1.73 &    ...  &    7.9  &    ...  &    ...  &   23.4  &    ...  &    ...  &    ...  &    ...  \\
 3856.37 &   26.0 &   0.05 &   $-$1.29 &   71.9  &   52.6  &   79.8  &   65.8  &   82.8  &    ...  &    ...  &   71.7  &    ...  \\
 3859.91 &   26.0 &   0.00 &   $-$0.71 &   91.9  &   85.9\tablenotemark{b} &  124.0  &   69.2  &  102.0  &    ...  &    ...  &  100.0  &    ...  \\
 3865.52 &   26.0 &   1.01 &   $-$0.98 &   39.3  &   27.3  &   43.8  &   39.3  &   47.7  &    ...  &    ...  &   41.4  &    ...  \\
 3878.02 &   26.0 &   0.96 &   $-$0.91 &   49.1  &   34.2  &   76.2  &   48.6  &   50.2  &    ...  &    ...  &   47.1  &    ...  \\
 3878.57 &   26.0 &   0.09 &   $-$1.38 &   68.8  &   48.4  &   76.2  &    ...  &   83.2  &    ...  &    ...  &   64.5  &    ...  \\
 3886.28 &   26.0 &   0.05 &   $-$1.08 &    ...  &    ...  &   90.5  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 3887.05 &   26.0 &   0.91 &   $-$1.14 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 3895.66 &   26.0 &   0.11 &   $-$1.67 &    ...  &    ...  &   71.1  &    ...  &   56.2  &    ...  &    ...  &   57.5  &    ...  \\
 3899.71 &   26.0 &   0.09 &   $-$1.53 &   61.8  &   43.3  &   64.3  &   65.5\tablenotemark{b} &   68.5  &    ...  &    ...  &   56.8  &    ...  \\
 3920.26 &   26.0 &   0.12 &   $-$1.75 &   51.4  &   35.8  &   47.4  &    ...  &   61.8  &    ...  &    ...  &   52.0  &    ...  \\
 3922.91 &   26.0 &   0.05 &   $-$1.65 &    ...  &   43.6  &   67.2  &   60.3  &   60.6  &    ...  &   95.6  &   59.1  &    ...  \\
 4005.24 &   26.0 &   1.56 &   $-$0.61 &   38.1  &   24.0  &    ...  &   25.5  &   51.7  &  109.0  &    ...  &   38.7  &    ...  \\
 4045.81 &   26.0 &   1.48 &    0.28 &   68.2  &   64.2  &   98.4  &   52.0  &   86.1  &    ...  &    ...  &   84.2  &    ...  \\
 4063.59 &   26.0 &   1.56 &    0.07 &   57.6  &   50.8  &   77.8  &   47.2  &   78.8  &    ...  &    ...  &   62.2  &    ...  \\
 4071.74 &   26.0 &   1.61 &   $-$0.02 &   63.2  &   49.7  &   87.8  &   42.3  &   69.2  &    ...  &    ...  &   71.4  &    ...  \\
 4076.63 &   26.0 &   3.21 &   $-$0.37 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4132.06 &   26.0 &   1.61 &   $-$0.67 &   35.7  &   20.5  &   60.8  &   24.8  &   44.5  &    ...  &    ...  &   34.8  &    ...  \\
 4134.68 &   26.0 &   2.83 &   $-$0.49 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4143.87 &   26.0 &   1.56 &   $-$0.46 &   37.1  &   31.4  &   57.8  &   30.8  &   51.3  &  120.5  &   88.3  &   41.8  &    ...  \\
 4147.67 &   26.0 &   1.48 &   $-$2.10 &    ...  &    ...  &    ...  &    ...  &    ...  &   64.7  &    ...  &    ...  &    ...  \\
 4156.80 &   26.0 &   2.83 &   $-$0.61 &   12.4  &    ...  &   58.6\tablenotemark{b} &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4181.76 &   26.0 &   2.83 &   $-$0.18 &    ...  &    ...  &    ...  &    ...  &   13.0  &    ...  &    ...  &    ...  &    ...  \\
 4187.04 &   26.0 &   2.45 &   $-$0.55 &   12.1  &    ...  &    ...  &    ...  &   16.4  &   76.2  &    ...  &    ...  &   75.4  \\
 4187.80 &   26.0 &   2.42 &   $-$0.55 &   15.6  &    ...  &   21.9  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4191.43 &   26.0 &   2.47 &   $-$0.73 &   15.8  &    ...  &    ...  &    ...  &    ...  &   67.6  &    ...  &    ...  &   80.2  \\
 4199.10 &   26.0 &   3.05 &    0.25 &   16.4  &   12.6  &    ...  &    ...  &   23.1  &    ...  &    ...  &   22.7  &    ...  \\
 4202.03 &   26.0 &   1.48 &   $-$0.70 &   40.9  &   25.0  &    ...  &    ...  &   50.7  &    ...  &    ...  &   40.1  &    ...  \\
 4222.21 &   26.0 &   2.45 &   $-$0.97 &    ...  &    ...  &    ...  &    ...  &    ...  &   49.8  &    ...  &    ...  &    ...  \\
 4227.43 &   26.0 &   3.33 &    0.23 &   10.6  &    ...  &    ...  &    ...  &   23.7  &   61.8  &    ...  &    ...  &    ...  \\
 4233.60 &   26.0 &   2.48 &   $-$0.60 &   14.0  &    ...  &   21.2  &    ...  &    ...  &   74.7  &   37.9  &    ...  &    ...  \\
 4250.12 &   26.0 &   2.47 &   $-$0.40 &   17.3  &    ...  &    ...  &    ...  &   22.5  &    ...  &    ...  &   14.5  &    ...  \\
 4260.47 &   26.0 &   2.40 &   $-$0.02 &   33.2  &   19.5  &   49.0  &   16.0  &   42.6  &  101.5  &   77.2  &   31.5  &    ...  \\
 4271.15 &   26.0 &   2.45 &   $-$0.35 &   17.3  &    ...  &   23.0  &    ...  &   23.9  &    ...  &    ...  &    ...  &    ...  \\
 4271.76 &   26.0 &   1.48 &   $-$0.16 &   57.4  &   45.9  &   67.4  &    ...  &   64.3  &    ...  &    ...  &   66.7  &    ...  \\
 4282.40 &   26.0 &   2.17 &   $-$0.82 &    ...  &    ...  &    ...  &    ...  &   17.0  &   80.5  &   54.9  &   13.1  &   84.4  \\
 4325.76 &   26.0 &   1.61 &   $-$0.01 &   52.8  &   50.3  &   67.1  &    ...  &   68.6  &    ...  &    ...  &   60.9  &    ...  \\
 4383.55 &   26.0 &   1.48 &    0.20 &   71.7  &   62.2  &   89.7  &   62.7  &   82.3  &    ...  &  132.5  &   76.6  &    ...  \\
 4404.75 &   26.0 &   1.56 &   $-$0.14 &   54.6  &    ...  &   74.7  &   43.0  &   68.9  &  118.5\tablenotemark{b} &    ...  &   61.1  &    ...  \\
 4415.12 &   26.0 &   1.61 &   $-$0.61 &   37.3  &   24.8  &    ...  &    ...  &   45.0  &  117.5  &    ...  &   37.1  &  110.5  \\
 4442.34 &   26.0 &   2.20 &   $-$1.25 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4447.72 &   26.0 &   2.22 &   $-$1.34 &    ...  &    ...  &    ...  &    ...  &    ...  &   53.3  &    ...  &    ...  &   58.5  \\
 4461.65 &   26.0 &   0.09 &   $-$3.20 &   12.9  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4466.55 &   26.0 &   2.83 &   $-$0.60 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4489.74 &   26.0 &   0.12 &   $-$3.97 &    ...  &    ...  &    ...  &    ...  &    ...  &   45.0  &   37.9\tablenotemark{b} &    ...  &   55.8  \\
 4494.56 &   26.0 &   2.20 &   $-$1.14 &    ...  &    ...  &    ...  &    ...  &   11.1  &   62.6  &   46.5  &    ...  &   61.4  \\
 4528.61 &   26.0 &   2.18 &   $-$0.82 &   14.0  &    ...  &   18.9  &    7.3 &   10.5  &   75.2  &   57.4  &    ...  &   82.2  \\
 4531.15 &   26.0 &   1.48 &   $-$2.15 &    ...  &    ...  &    ...  &    ...  &    ...  &   55.3  &    ...  &    ...  &   56.4  \\
 4871.32 &   26.0 &   2.87 &   $-$0.36 &    ...  &    ...  &    ...  &    ...  &    ...  &   62.2  &   51.3  &    ...  &   62.5  \\
 4872.14 &   26.0 &   2.88 &   $-$0.57 &    ...  &    ...  &    ...  &    ...  &    ...  &   49.1  &    ...  &    ...  &    ...  \\
 4891.49 &   26.0 &   2.85 &   $-$0.11 &   11.4  &    ...  &    ...  &    ...  &   22.5  &   72.2  &   56.5  &    ...  &   77.1  \\
 4903.31 &   26.0 &   2.88 &   $-$0.93 &    ...  &    ...  &    ...  &    ...  &    ...  &   30.0  &   16.1  &    ...  &    ...  \\
 4918.99 &   26.0 &   2.87 &   $-$0.34 &    ...  &    ...  &    ...  &    ...  &   23.3  &   56.4  &   39.9  &    ...  &   72.2  \\
 4920.50 &   26.0 &   2.83 &    0.07 &    ...  &   12.1  &    ...  &    6.1 &   26.8  &   71.1  &   59.3  &    ...  &    ...  \\
 4939.69 &   26.0 &   0.86 &   $-$3.34 &    ...  &    ...  &    ...  &   19.3\tablenotemark{b} &    ...  &    ...  &    ...  &    ...  &    ...  \\
 4994.13 &   26.0 &   0.92 &   $-$3.08 &    ...  &    ...  &    ...  &    ...  &    ...  &   53.8  &   18.4  &    ...  &   52.2  \\
 5006.12 &   26.0 &   2.83 &   $-$0.62 &    ...  &    ...  &    ...  &    ...  &    ...  &   32.0  &   22.5  &    ...  &    ...  \\
 5041.76 &   26.0 &   1.49 &   $-$2.20 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5051.64 &   26.0 &   0.92 &   $-$2.80 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  \\
 5083.34 &   26.0 &   0.96 &   $-$2.96 &    ...  &    ...  &    ...  &    ...  &    ...  &   51.1  &    ...  &    ...  &    ...  \\
 5123.72 &   26.0 &   1.01 &   $-$3.07 &    ...  &    ...  &    ...  &    ...  &    ...  &   48.3  &    ...  &    ...  &   46.3  \\
 5127.36 &   26.0 &   0.92 &   $-$3.31 &    ...  &    ...  &    ...  &    ...  &    ...  &   53.8  &    ...  &    ...  &   32.7  \\
 5150.84 &   26.0 &   0.99 &   $-$3.04 &    ...  &    ...  &    ...  &    ...  &    ...  &   40.3  &    ...  &    ...  &   48.5  \\
 5166.28 &   26.0 &   0.00 &   $-$4.20 &    ...  &    ...  &    ...  &    ...  &    ...  &   59.9  &    ...  &    ...  &   66.2  \\
 5171.60 &   26.0 &   1.49 &   $-$1.79 &    ...  &    ...  &    ...  &    ...  &    ...  &   87.8  &    ...  &    ...  &   82.8  \\
 5191.46 &   26.0 &   3.04 &   $-$0.55 &    ...  &    ...  &    ...  &    ...  &    ...  &   38.3  &   39.2  &    ...  &   57.9  \\
 5192.34 &   26.0 &   3.00 &   $-$0.42 &    ...  &    ...  &    ...  &    ...  &    ...  &   42.1  &   39.2  &    ...  &   63.6  \\
 5194.94 &   26.0 &   1.56 &   $-$2.09 &    ...  &    ...  &    ...  &    ...  &    ...  &   66.0  &   41.3  &    ...  &    ...  \\
 5216.27 &   26.0 &   1.61 &   $-$2.15 &    ...  &    ...  &    ...  &    ...  &    ...  &   50.2  &   25.0  &    ...  &    ...  \\
 5232.94 &   26.0 &   2.94 &   $-$0.06 &    ...  &    ...  &    ...  &    ...  &   15.7  &   77.8  &   65.1  &    ...  &   88.5  \\
 5266.56 &   26.0 &   3.00 &   $-$0.39 &    ...  &    ...  &    ...  &    ...  &    ...  &   54.3  &   34.8  &    ...  &   47.7  \\
 5269.54 &   26.0 &   0.86 &   $-$1.32 &   45.0  &   25.5  &   46.7  &   43.6  &   62.0  &  129.0  &   89.2  &   46.7  &  159.0  \\
 5281.79 &   26.0 &   3.04 &   $-$0.83 &    ...  &    ...  &    ...  &    ...  &    ...  &   32.1  &   28.9  &    ...  &    ...  \\
 5283.62 &   26.0 &   3.24 &   $-$0.52 &    ...  &    ...  &    ...  &    ...  &    ...  &   36.5  &    ...  &    ...  &   50.2  \\
 5324.18 &   26.0 &   3.21 &   $-$0.24 &    ...  &    ...  &    ...  &    ...  &   13.0  &   62.1  &   59.1\tablenotemark{b} &    ...  &   50.8  \\
 5328.04 &   26.0 &   0.92 &   $-$1.47 &   42.5  &   21.3  &    ...  &   37.8  &   45.0  &  120.5  &   81.6  &   41.0  &  149.5  \\
 5328.53 &   26.0 &   1.56 &   $-$1.85 &    ...  &    ...  &    ...  &    ...  &    ...  &   86.9  &   48.8  &    ...  &   82.2  \\
 5371.49 &   26.0 &   0.96 &   $-$1.65 &   41.0  &   10.4  &    ...  &   23.6  &   33.2  &  112.0  &   81.8  &   37.2  &  146.0  \\
 5397.13 &   26.0 &   0.92 &   $-$1.99 &    ...  &    ...  &    ...  &   18.0  &   19.0  &  111.0  &   64.4  &    ...  &  107.5  \\
 5405.78 &   26.0 &   0.99 &   $-$1.84 &    ...  &    9.1  &    ...  &   17.2  &   20.5  &  123.0  &   67.8  &    ...  &  108.5  \\
 5429.70 &   26.0 &   0.96 &   $-$1.88 &    ...  &    ...  &    ...  &   16.2  &    ...  &  110.0  &   67.8  &    ...  &  104.0  \\
 5434.52 &   26.0 &   1.01 &   $-$2.12 &    ...  &    ...  &    ...  &   11.9  &   19.0  &   88.4  &    ...  &    ...  &   78.5  \\
 5446.92 &   26.0 &   0.99 &   $-$1.91 &    ...  &    ...  &    ...  &   20.2  &    ...  &   97.1  &   57.2  &   19.3  &   99.4  \\
 5455.61 &   26.0 &   1.01 &   $-$2.09 &    ...  &    ...  &    ...  &   13.1  &   18.4  &  109.0  &   65.2  &    ...  &  130.0\tablenotemark{b} \\
 5497.52 &   26.0 &   1.01 &   $-$2.85 &    ...  &    ...  &    ...  &    ...  &    ...  &   56.8  &    ...  &    ...  &   76.7  \\
 5501.47 &   26.0 &   0.96 &   $-$3.05 &    ...  &    ...  &    ...  &    ...  &    ...  &   85.2\tablenotemark{b} &    ...  &    ...  &   55.8  \\
 5506.78 &   26.0 &   0.99 &   $-$2.80 &    ...  &    ...  &    ...  &    ...  &    ...  &   66.6  &    ...  &    ...  &   72.8  \\
 5572.84 &   26.0 &   3.40 &   $-$0.31 &    ...  &    ...  &    ...  &    ...  &    ...  &    ...  &   40.2  &    ...  &   46.2  \\
 5586.76 &   26.0 &   3.37 &   $-$0.14 &    ...  &    ...  &    ...  &    ...  &    ...  &   53.0  &    ...  &    ...  &   49.0  \\
 5615.64 &   26.0 &   3.33 &   $-$0.14 &    ...  &    ...  &   27.5\tablenotemark{b} &    ...  &    ...  &   60.2  &   28.5  &    ...  &   64.4  \\
 6136.62 &   26.0 &   2.45 &   $-$1.40 &    ...  &    ...  &    ...  &    ...  &    ...  &   47.8  &    ...  &    ...  &   48.8  \\
 6137.69 &   26.0 &   2.59 &   $-$1.40 &    ...  &    ...  &    ...  &    ...  &    ...  &   31.8  &    ...  &    ...  &   40.2  \\
 6191.56 &   26.0 &   2.43 &   $-$1.42 &    ...  &    ...  &    ...  &    ...  &    ...  &   30.5  &    ...  &    ...  &   42.6  \\
 6230.72 &   26.0 &   2.56 &   $-$1.28 &    ...  &    ...  &    ...  &    ...  &    ...  &   42.8  &    ...  &    ...  &   51.2  \\
 6252.56 &   26.0 &   2.40 &   $-$1.69 &    ...  &    ...  &    ...  &    ...  &    ...  &   31.5  &    ...  &    ...  &   32.8  \\
 6393.60 &   26.0 &   2.43 &   $-$1.58 &    ...  &    ...  &    ...  &    ...  &    ...  &   35.6  &    ...  &    ...  &   47.8  \\
 6494.98 &   26.0 &   2.40 &   $-$1.27 &    ...  &    ...  &    ...  &    ...  &    ...  &   54.1  &   57.8\tablenotemark{b} &    ...  &   58.3  \\
 4178.86 &   26.1 &   2.58 &   $-$2.50 &    ...  &    ...  &    ...  &    ...  &   13.7  &    ...  &    ...  &    ...  &    ...  \\
 4233.17 &   26.1 &   2.58 &   $-$1.90 &   15.4  &    ...  &   31.6  &    ...  &   17.0  &    ...  &    ...  &   14.8  &    ...  \\
 4508.29 &   26.1 &   2.86 &   $-$2.25 &    ...  &    ...  &    ...  &    ...  &   11.1  &   36.4  &   21.0  &    ...  &    ...  \\
 4520.22 &   26.1 &   2.81 &   $-$2.60 &    ...  &    ...  &    ...  &    ...  &    ...  &   28.8  &   18.4  &    ...  &    ...  \\
 4522.63 &   26.1 &   2.84 &   $-$2.03 &    ...  &    ...  &    ...  &    6.9 &   15.6  &   49.5  &   45.4  &    ...  &   56.0  \\
 5197.58 &   26.1 &   3.23 &   $-$2.23 &    ...  &    ...  &    ...  &    ...  &    ...  &   27.5  &    ...  &    ...  &    ...  \\
 5234.63 &   26.1 &   3.22 &   $-$2.15 &    ...  &    ...  &    ...  &    ...  &    ...  &   25.5  &    ...  &    ...  &   54.1  \\
 3845.46 &   27.0 &   0.92 &    0.01 &    ...  &    ...  &    ...  &   15.1  &    ...  &   79.3  &    ...  &    ...  &    ...  \\
 3995.30 &   27.0 &   0.92 &   $-$0.22 &    ...  &    ...  &    ...  &    ...  &    ...  &   78.5  &   53.6  &    ...  &    ...  \\
 4118.77 &   27.0 &   1.05 &   $-$0.49 &    ...  &    5.0  &    ...  &    ...  &    ...  &   67.1  &    ...  &    ...  &    ...  \\
 4121.31 &   27.0 &   0.92 &   $-$0.32 &    ...  &    ...  &    ...  &    ...  &    ...  &   76.6  &    ...  &    ...  &    ...  \\
 3807.14 &   28.0 &   0.42 &   $-$1.18 &   31.3  &    8.9  &    ...  &   26.5  &    ...  &   85.7  &    ...  &   20.6  &    ...  \\
 3858.29 &   28.0 &   0.42 &   $-$0.97 &   43.2  &   21.0  &    ...  &   30.0  &   30.5  &   99.0  &    ...  &   35.9  &    ...  \\
 5476.90 &   28.0 &   1.83 &   $-$0.89 &    ...  &    ...  &    ...  &    ...  &   10.9  &   52.7  &   26.4  &    ...  &   88.8  \\
 4077.71 &   38.1 &   0.00 &    0.16 &    ...  &   12.4  &   79.2  &   25.7  &   37.2  &  145.0  &    62.5  &   33.4  &  $<$143.0  \\
 4215.52 &   38.1 &   0.00 &   $-$0.16 &    ...  &    7.2  &   53.3  &   16.0  &   24.5  &  116.5  &    ...  &   24.5  &    ...  \\
 4554.03 &   56.1 &   0.00 &    0.16 &    ...  &    ...  &   24.4  &    ...  &    ...  &   86.5  &   18.1  &    ...  &   85.0  \\
 4934.08 &   56.1 &   0.00 &   $-$0.15 &    ...  &    ...  &    ...  &    ...  &    ...  &   85.8  &    9.0  &    ...  &   50.5  \\
 6141.73 &   56.1 &   0.70 &   $-$0.08 &    ...  &    ...  &    ...  &    ...  &    ...  &   33.5  &    ...  &    ...  &   35.0  \\
 6496.91 &   56.1 &   0.60 &   $-$0.38 &    ...  &    ...  &    ...  &    ...  &    ...  &   27.4  &    ...  &    ...  &   19.8  \\
\enddata                                                                                                                
\tablenotetext{a}{$S/N$ per $\sim$0.17\,{\AA}~pixel at 4500\,{\AA}}                                                      
\tablenotetext{b}{These lines produce discrepant abundances and are not included in the results reported in Paper II}   
\end{deluxetable}                                                                                                       
\end{center}                                                                                                          



==> tab8.tex <==
\begin{deluxetable}{lccr}
\tabletypesize{\tiny}
\tablecolumns{4} 
\tablewidth{0pc} 
\tablecaption{\label{Tab:individual_velocities} INDIVIDUAL RADIAL VELOCITIES \label{tab:rvs2}} 
\tablehead{ 
\colhead{Star} & 
\colhead{Telescope\tablenotemark{a}/Date} & 
\colhead{Julian Date} & 
\colhead{V$_{\rm r}$\tablenotemark{b}} \\ 
\colhead{} & 
\colhead{} & 
\colhead{} & 
\colhead{(km s$^{-1}$)}\\  
\colhead{(1)} & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} 
}
\startdata 
52972-1213-507 & K Nov07 & 2454437.06233 & $-$176.6 \\
 & K Nov07 & 2454437.07710 & $-$177.3 \\
53327-2044-515 & K Nov07 & 2454435.94873 & $-$193.7 \\
 & K Nov07 & 2454436.81393 & $-$193.1 \\
 & K Nov07 & 2454436.85729 & $-$193.7 \\
53436-1996-093 & K Nov07 & 2454437.09230 & $-$11.0 \\
 & K Nov07 & 2454437.10709 & $-$15.6 \\
 & K Nov07 & 2454437.13194 & $-$16.4 \\
 & K Nov07 & 2454437.14671 & $-$18.0 \\
 & K Mar08 & 2454552.81982 & $-$17.7 \\
 & K Mar08 & 2454552.83460 & $-$17.2 \\
 & K Mar08 & 2454552.84936 & $-$15.2 \\
 & K Mar08 & 2454552.86414 & $-$17.7 \\
 & K Mar08 & 2454552.87893 & $-$17.9 \\
 & K Mar08 & 2454552.89371 & $-$18.6 \\
 & K Mar08 & 2454552.90849 & $-$17.7 \\
 & K Mar08 & 2454552.92328 & $-$16.6 \\
 & K Mar08 & 2454552.93807 & $-$16.2 \\
 & K Mar08 & 2454552.95283 & $-$17.3 \\
 & K Mar08 & 2454552.96762 & $-$17.5 \\
54142-2667-094 & K Nov07 & 2454437.03189 & 42.9 \\
 & K Nov07 & 2454437.04671 & 43.9 \\
BS~16545-089 & K Mar08 & 2454551.77746 & $-$160.4 \\
 & K Mar08 & 2454551.79919 & $-$161.4 \\
 & K Mar08 & 2454551.82095 & $-$161.7 \\
CS~30336-049 & M Jun07 & 2454274.84090 & $-$237.9 \\
 & M Jun07 & 2454275.78996 & $-$236.2 \\
 & M Jun07 & 2454275.81521 & $-$235.8 \\
HE~0049--3948 & M Dec07 & 2454456.55349 & 190.7 \\
 & M Dec07 & 2454456.58345 & 191.4 \\
 & M Dec07 & 2454456.59843 & 190.0 \\
 & M Dec07 & 2454456.61339 & 190.1 \\
 & M Dec07 & 2454457.56454 & 191.2 \\
 & M Dec07 & 2454457.58646 & 193.2 \\
 & M Dec07 & 2454457.60836 & 189.9 \\
 & M Dec07 & 2454457.63028 & 190.2 \\
 & M Sep08 & 2454716.76612 & 188.2 \\
 & M Sep08 & 2454716.84034 & 191.1 \\
 & M Sep08 & 2454716.85531 & 190.9 \\
 & M Sep08 & 2454716.87026 & 188.2 \\
 & M Sep08 & 2454717.86276 & 193.6 \\
 & M Sep08 & 2454717.87778 & 191.9 \\
HE~0057--5959 & M Jun07 & 2454272.83040 & 374.4 \\
 & M Jun07 & 2454272.86089 & 375.7 \\
 & M Jun07 & 2454272.88280 & 373.3 \\
 & M Jun07 & 2454272.90681 & 372.7 \\
 & M Jun07 & 2454273.83825 & 373.8 \\
 & M Jun07 & 2454273.86018 & 374.7 \\
 & M Jun07 & 2454273.88212 & 375.4 \\
 & M Jun07 & 2454273.90405 & 375.2 \\
 & M Jun07 & 2454274.85992 & 379.4 \\
 & M Jun07 & 2454275.83670 & 374.8 \\
 & M Jun07 & 2454275.85861 & 377.5 \\
 & M Jun07 & 2454275.88060 & 376.4 \\
 & M Jun07 & 2454275.90251 & 375.9 \\
HE~0102--1213 & K Nov07 & 2454436.77982 & 90.5 \\
HE~0146--1548 & K Nov07 & 2454436.87161 & $-$114.8 \\
 & K Nov07 & 2454436.88642 & $-$115.1 \\
HE~0207--1423 & K Nov07 & 2454436.90406 & $-$209.8 \\
 & K Nov07 & 2454436.91654 & $-$209.4 \\
HE~0228--4047 & M Dec07 & 2454456.62998 & 122.1 \\
 & M Dec07 & 2454456.64495 & 123.9 \\
 & M Dec07 & 2454456.65992 & 123.8 \\
 & M Dec07 & 2454456.67489 & 121.9 \\
 & M Dec07 & 2454456.68986 & 126.3 \\
 & M Dec07 & 2454457.65390 & 123.2 \\
 & M Dec07 & 2454457.67582 & 125.4 \\
 & M Dec07 & 2454457.69773 & 125.8 \\
 & M Dec07 & 2454457.71965 & 122.1 \\
 & M Sep08 & 2454717.89167 & 129.5 \\
 & M Sep08 & 2454717.90661 & 127.4 \\
HE~0231--6025 & M Dec07 & 2454456.70367 & 296.6 \\
HE~0253--1331 & K Nov07 & 2454436.93006 & 24.8 \\
 & K Nov07 & 2454436.94256 & 25.5 \\
 & K Nov07 & 2454435.96501 & 41.4 \\
HE~0314--1739 & K Nov07 & 2454436.95594 & 41.3 \\
 & K Nov07 & 2454436.97072 & 40.1 \\
HE~0355--3728 & M Dec07 & 2454456.72133 & 83.3 \\
 & M Dec07 & 2454456.73629 & 80.7 \\
HE~0945--1435 & K Mar08 & 2454551.73082 & 120.7 \\
 & K Mar08 & 2454551.75258 & 122.1 \\
 & K Mar08 & 2454552.72728 & 122.6 \\
 & K Mar08 & 2454552.74206 & 121.8 \\
 & K Mar08 & 2454552.75684 & 120.2 \\
 & K Mar08 & 2454552.77162 & 122.1 \\
 & K Mar08 & 2454552.78640 & 122.7 \\
 & K Mar08 & 2454552.80117 & 121.8 \\
HE~1055+0104 & K Nov07 & 2454437.12214 & 324.6 \\
HE~1116--0054 & M Jun07 & 2454274.47618 & 147.8 \\
 & M Jun07 & 2454274.49810 & 150.7 \\
 & M Jun07 & 2454274.52002 & 149.1 \\
 & M Jun07 & 2454274.54195 & 148.8 \\
 & K Nov07 & 2454436.12281 & 147.4 \\
 & K Nov07 & 2454436.13760 & 149.2 \\
 & M Dec07 & 2454456.78524 & 149.2 \\
 & M Dec07 & 2454456.80716 & 148.3 \\
 & M Dec07 & 2454456.82909 & 150.1 \\
 & M Dec07 & 2454457.79451 & 151.1 \\
 & M Dec07 & 2454457.81643 & 147.6 \\
 & K Mar08 & 2454551.84513 & 146.3 \\
 & K Mar08 & 2454551.86690 & 149.0 \\
 & K Mar08 & 2454551.88864 & 147.9 \\
 & K Mar08 & 2454551.91039 & 149.8 \\
 & K Mar08 & 2454551.93214 & 147.5 \\
 & K Mar08 & 2454551.95393 & 148.0 \\
 & K Mar08 & 2454552.98952 & 151.9 \\
 & K Mar08 & 2454553.00432 & 145.7 \\
HE~1142--1422 & M Jun07 & 2454273.49861 & $-$102.5 \\
 & M Jun07 & 2454273.52084 & $-$102.0 \\
HE~1201--1512 & M Jun07 & 2454272.47807 & 238.7 \\
 & M Jun07 & 2454272.50505 & 238.9 \\
 & K Mar08 & 2454551.98076 & 237.2 \\
 & K Mar08 & 2454552.00248 & 237.3 \\
HE~1204--0744 & M Jun07 & 2454273.53278 & $-$52.3 \\
 & M Jun07 & 2454273.55553 & $-$51.5 \\
 & M Jun07 & 2454273.57751 & $-$45.3 \\
HE~1207--3108 & M Jun07 & 2454273.46864 & $-$3.7 \\
HE~1320--2952 & M Jun07 & 2454272.53051 & 390.0 \\
 & K Mar08 & 2454553.02472 & 389.3 \\
 & K Mar08 & 2454553.03589 & 391.5 \\
 & K Mar08 & 2454553.05067 & 389.3 \\
HE~1346--0427 & K Mar08 & 2454552.02679 & $-$47.6 \\
 & K Mar08 & 2454552.04853 & $-$47.9 \\
 & K Mar08 & 2454552.07026 & $-$47.9 \\
HE~1402--0523 & M Jun07 & 2454272.54638 & $-$68.9 \\
 & M Jun07 & 2454272.56830 & $-$68.6 \\
HE~1506--0113 & V Jul08 & 2454650.63069 & $-$137.1 \\
 & V Jul08 & 2454651.62859 & $-$136.9 \\
 & V Jul08 & 2454653.51893 & $-$136.9 \\
 & V Jul08 & 2454672.48673 & $-$137.6 \\
HE~2020--5228 & M Jun07 & 2454273.75335 & $-$39.9 \\
 & M Jun07 & 2454273.77527 & $-$43.0 \\
HE~2032--5633 & M Jun07 & 2454272.72175 & 260.4 \\
HE~2047--4421 & M Jun07 & 2454273.71477 & 25.9 \\
HE~2135--1924 & K Nov07 & 2454436.71514 & $-$251.8 \\
 & K Nov07 & 2454436.73345 & $-$254.0 \\
HE~2136--6030 & M Jun07 & 2454273.77908 & 154.5 \\
 & M Jun07 & 2454273.79872 & 158.4 \\
HE~2139--5432 & M Dec07 & 2454457.51872 & 112.3 \\
 & M Dec07 & 2454457.53024 & 113.6 \\
 & M Dec07 & 2454457.54173 & 114.3 \\
 & M Sep08 & 2454716.48660 & 115.5 \\
 & M Sep08 & 2454716.50158 & 115.0 \\
 & M Sep08 & 2454716.51659 & 116.3 \\
 & M Sep08 & 2454716.53849 & 114.9 \\
 & M Sep08 & 2454716.56041 & 114.7 \\
 & M Sep08 & 2454716.58231 & 116.7 \\
 & M Sep08 & 2454716.60564 & 116.0 \\
 & M Sep08 & 2454716.62756 & 115.2 \\
 & M Sep08 & 2454716.64946 & 112.4 \\
 & M Sep08 & 2454716.67279 & 115.1 \\
 & M Sep08 & 2454716.69470 & 115.8 \\
 & M Sep08 & 2454716.71660 & 114.0 \\
 & M Sep08 & 2454716.73850 & 114.7 \\
 & M Sep08 & 2454717.71090 & 120.9 \\
HE~2141--0726 & K Nov07 & 2454436.74605 & $-$38.1 \\
 & K Nov07 & 2454436.76085 & $-$38.2 \\
HE~2142--5656 & M Jun07 & 2454272.74315 & 103.4 \\
HE~2202--4831 & M Jun07 & 2454272.75521 & 56.0 \\
 & M Jun07 & 2454272.77715 & 56.4 \\
HE~2246--2410 & M Jun07 & 2454273.80873 & $-$1.8 \\
 & M Jun07 & 2454273.82717 & $-$4.4 \\
HE~2247--7400 & M Jun07 & 2454272.82002 & 5.7\\ 
\enddata 
\tablenotetext{a}{K = Keck, M = Magellan, V = VLT}
\tablenotetext{b}{Heliocentric radial velocity}
\end{deluxetable} 


